Towards Query Optimization for SPARQL Property Paths

The extension of SPARQL in version 1.1 with property paths offers a type of regular path query for RDF graph databases. Such queries are difficult to optimize and evaluate efficiently, however. We have embarked on a project, Waveguide, to build a cost-based optimizer for SPARQL queries with property paths. Waveguide builds a query plan - a waveguide plan (WGP) - which guides the query evaluation. There are numerous choices in the construction of a plan, and a number of optimization methods, meaning the space of plans for a query can be quite large. Execution costs of plans for the same query can vary by orders of magnitude. We illustrate the types of optimizations this approach affords and the performance gains that can be obtained. A WGP's costs can be estimated, which opens the way to cost-based optimization.

==> abs.tex <==
%!TEX root = paper.tex

%============================================================================%
\begin{abstract}
\label{sec:abstract}

The extension of \sparql\ in version 1.1 with \emph{property paths} 
offers a type of {\em regular path query}
for \rdf\ graph databases.
% While eminently useful,
Such queries are difficult to optimize and evaluate efficiently,
however.
We have embarked on a project, \waveguide,
to build a cost-based optimizer
for \sparql\ queries with property paths.
%
\waveguide\ builds a query plan---%
a \emph{waveguide plan} (\wgp)---%
which \emph{guides} the query evaluation.
There are numerous choices in the construction of a plan,
and a number of optimization methods,
meaning the space of plans for a query can be quite large.
Execution costs of plans for the same query can vary
by orders of magnitude.
% with the best plan often offering excellent performance.
%
We illustrate
the types of optimizations this approach affords
and the performance gains that can be obtained.
A \wgp's costs can be estimated,
which opens the way to cost-based optimization.

% Regular path queries (RPQs) are a powerful navigational mechanism
% in graph databases.
% Recently,
% there has been renewed interest in such queries
% in the context of the Semantic Web.
% In this work,
% we propose Waveguide,
% a novel RPQ evaluation strategy that is based
% on a fusion of an iterative search and dynamic programming.
% This demonstration is designed to achieve three goals.
% First,
% we show the practical feasibility of the Waveguide approach
% in the context of current Semantic Web and relational technologies.
% Second,
% we visualize the key steps of the evaluation process
% in order to familiarize the researchers with our approach.
% Finally,
% we provide an interactive demonstration of query evaluation scenarios
% in Social Networks and Life Sciences domains
% to highlight the interesting challenges involved
% in the proposed evaluation strategy.

%----------------------------------------------------------------------------%
\end{abstract}



==> background.tex <==
%!TEX root = paper.tex
%============================================================================%
\begin{Sect}{Background \& Related Work}
\label{SEC/bg}

In \S\ref{SEC/bg/RPQs},
we provide relevant background on path queries.
%
The literature on path queries over graphs,
as is pertinent to property paths,
comes from two distinct sources:

\begin{enumerate}
\item \label{point: rqp work}
	work on \emph{regular path queries} (\rpq s);
	and

\item \label{point: property-path work}
	work on \sparql\ platforms to extend to version 1.1
	to handle \emph{property paths}.

\end{enumerate}

Research on \rpq s,
which well precedes \rdf\ and \sparql,
mostly focused on theoretical aspects,
but little on performance issues
for evaluating such queries in practice.%
\footnote{%
	Regular-path queries have been considered under both
	\emph{simple}- and \emph{arbitrary}-path semantics.
	Under simple-path semantics,
	a path in the graph to match must not repeat any nodes;
	under arbitrary-path semantics,
	they may.
	\sparql\ adopts \emph{arbitrary}-path semantics,
	for the sake of tractability.
}
The seminal work
that introduced the \textsf{G+} query language
\cite{mendelzon1995finding}
exploited the natural observation
that where there is a regular expression,
there is a \emph{finite automaton} (\textsf{FA})
that is a \emph{recognizer} for it.
They showed how to use finite state machines
to direct search over the graph
to evaluate a \rpq.
In essence,
an FA corresponding to the query's regular expression
provides a plan for its evaluation.
Subsequent work on \rpq s followed on this idea.
%
Let us call this the \fa\ approach.
We overview this approach in \S\ref{SEC/bg/auto}.

% Something on simple vs arbitrary paths here...

Work on evaluating property paths---%
much newer by virtue of the fact that the \sparql\ 1.1 standard
is quite recent---%
meanwhile has mirrored
the dynamic-programming approach
behind the algorithm presented in the seminal work of
\cite{losemann2012complexity}.
This can be modeled by an extended \emph{relational algebra}
(\textsf{RA})
that includes an operator \(\alpha\) for \emph{transitive closure}
(\ara)
\cite{agrawal1988alpha}.
% \cite{abiteboul1995foundations}. % the "Alice" book.  NO!  That's WHILE
%
Let us call this the \ara\ approach.

As with the \fa\ approach for \rpq s,
\ara\ suffices for evaluating property paths.
The full power of relational algebra,
as extended with \(\alpha\),
can then be employed to devise an evaluation plan---%
an \ara-expression tree---%
based on the regular expression of the property path.
This general approach is found behind many \sparql\ platforms,
as it follows relational techniques well.
%
For example,
\virtuoso\
\cite{erling2010virtuoso},
a leading \sparql\ system
which is also a well-established relational database system,
extended their platform to accommodate property paths
by adding an ``\(\alpha\)'' operator to the engine.
%
We present this approach and characterize it by \ara\
in \S\ref{SEC/bg/DP-based}.

Work on property-path evaluation has been remiss
in not drawing the connection to \rpq s.
How do the \fa\ and \ara\ approaches compare?
Does one subsume the other?
Or are they \emph{incomparable}?
The latter is, in fact, the case,
and we show this in \S\ref{SEC/bg/plan_space}.
%
Furthermore,
a combined approach might be superior.
We show that it is in \S\ref{sec:eval}.

% How no one has been thinking about plans explicitly...

Both the \fa\ and \ara\ approaches
effectively provide evaluation plans for property-path queries.
However,
the \emph{plan spaces} that are implicit in these approaches
have not been considered.
In \fa,
choosing a different (but still correct) automaton
for the plan might offer a significantly more efficient plan.
In systems taking the \ara\ approach,
limited planning is sometimes done,
but not in a formal way to enumerate through the plan space
to find a best estimated plan,
as is done in relational systems.
We address this in \S\ref{sec:CoP}.

% We present brief background on
% 	regular path queries,
% 	their evaluation strategies
% and the related work with respect to each.

% We group RPQ evaluation strategies into two categories. 
% Algorithms in the first group utilize finite state machines 
% to aid the evaluation of a given RPQ 
% and are inspired by the algorithm 
% used in the implementation
% of the \textbf{G+} query language
% \cite{mendelzon1995finding}.
% Methods in the second group 
% use a dynamic programming approach inspired
% by the algorithm
% in \cite{losemann2012complexity}. 
% We provide details in the following subsections.

%----------------------------------------------------------------------------%
\begin{Sect}{Path Queries on Graphs}
\label{SEC/bg/RPQs}

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% graph databases

% A {\em graph database} is
% a finite, directed, edge-labeled graph.
A \emph{graph database} \(G\) can be defined as
\tuple{N, \Sigma, E}\
for which
	\(N\) is a finite set of nodes (vertices),
	\(\Sigma\) is a finite {\em alphabet} (a set of {\em labels}),
		and
	\(E\) is a set of {\em directed, labeled edges},
		\(E \subseteq N \times \Sigma \times N\).

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% a path and a path induced string (a label)

A {\em path} in a graph is defined as a sequence
\(p = n_0\)\-%
	\(a_0\)\-%
	\(n_1\)\-%
	\(\ldots\)\-%
	\(n_{k-1}\)\-%
	\(a_{k-1}\)\-%
	\(n_k\)
such that \(n_i \in N\),
	for \(0 \le i \le k\),
and \(\tuple{n_{i}, a_{i}, n_{i+1}} \in E\),
	for \(0 \le i < k\).
The path-induced \emph{path label} \(\lambda(p)\) is
the string
	\(a_1\)\-%
	\(a_2\)\-%
	\(\ldots\)\-%
	\(a_k\)%
	\(\in \Sigma^{*}\)
(for which \(\Sigma^{*}\) is a set of all finite strings
formed over \(\Sigma\)).
%
Each node \(n \in N\) is associated
with an {\em empty path}, \(n\),
the path label of which is the empty string,
denoted by \(\epsilon\).
%
% A {\em simple path} may not list the same node twice;
% an {\em arbitrary path} may.

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% a regular language

A \emph{regular expression} over alphabet \(\Sigma\) is defined inductively,
as follows:
	1.~the empty string \(\epsilon\) and each symbol \(r\in\Sigma\);
		and,
	2.~given regular expressions \(r\), \(r_1\), and \(r_2\),
		then
		(a) the concatenation \(r_1 r_2\),
		(b) the disjunction \(r_1 | r_2\),
			and
		(c) Kleene star \(r*\).
%
% \noindent
The \emph{regular language} defined by
the regular expression \(r\) is denoted by \(L(r)\).
Regular language is defined inductively,
as follows:
	1.~\(L(\epsilon) = \{ \epsilon \}\)
		and
		\(L(a) = \{ a \}\), for each \(a\in\Sigma\);
		and,
	2.~for inductively combining strings,
		(a) \(L(r_1 r_2) = L(r_1) \cdot L(r_2)\),
		(b) \(L(r_1 | r_2) = L(r_1) \cup L(r_2)\),
			and
		(c) \(L(r*) = \{ \epsilon \} \cup \bigcup_{i=1}^{\infty} L(r)^i\).

% \noindent
% Operator ``\(\cdot\)'' is string concatenation.
% \(L(r)^i\) denotes
% 	\(L(r)\)\-%
% 	\(\cdot\)\-%
% 	\(L(r)\)\-%
% 	\(\cdot\)\-%
% 	\(\ldots\)\-%
% 	\(\cdot\)\-%
% 	\(L(r)\),
% 	\(i\) times.
% \(\mbox{REG}(\Sigma)\) denotes
% the set of nonempty regular languages
% over \(\Sigma\).

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% path matching

%%% Do we need this?

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% RPQs

% A simple form of path query on graphs is
% the \emph{regular path query} (\rpq).
% RPQs have been well studied
% \cite{}.
%
A \emph{regular path query} \(Q\) is a tuple \tuple{x, r, y}\
for which \(x\) and \(y\) are free variables
(that range over nodes)
and \(r\) is a regular expression.
%
An {\em answer} to \(Q\) over graph \(G = \tuple{N, \Sigma, E}\)
is a pair \(\tuple{s,t}\in N \times N\)
such that there exists an arbitrary path \(p\)
from node \(s\) to node \(t\)
for which the path label \(\lambda(p)\) is in language \(L(r)\)
(\(\lambda(p)\in L(r)\)).
% \footnote{%
% 	\rpq s defined over {\em simple} paths
% 	have also been well studied.
% 	Our focus is on arbitrary paths.
% }
%
The {\em answer set} of \(Q\) over graph \(G\)
is the set of all answers of \(Q\) over \(G\).

%----------------------------------------------------------------------------%
% related work on RPQs

% \noindent
% RELATED WORK

Regular path queries
have been considered since \emph{semi-structured} data models
were first introduced
\cite{%
	abiteboul1997lorel,%
%	buneman1996query,%
%	florescu1998database,%
	mendelzon1995finding%,
}.
The complexity of \rpq s for graph databases
particularly has been well studied
\cite{%
	barcelo2012expressive,%
	calvanese1999rewriting%,
}.
% \emph{%
% 	Small bit more to cite a couple
% 	of the closest related \sparql\ works\ldots
% }
In \cite{koschmieder2012regular},
the idea of employing \nfa s to guide search
for \rpq\ evaluation appears.
In \cite{gubichev2013sparqling},
they perform a fixpoint evaluation for property paths.
In \cite{DBLP:conf/amw/YakovetsGG13},
we present a precursor of \waveguide\
that explores fixpoint evaluation for property paths
using \sql\ recursion.

%----------------------------------------------------------------------------%
% establishing a running example of a path query

% (figure: example of conversion of a property path to an NFA)
\begin{figure}
	\centering
	\input{eg_graph.tikz}
	%\includegraphics[width=.4\textwidth]{graph_eg.png}
	\caption{An example graph database.}
	\label{fig:graph_eg}
\end{figure}
% (end)

Regular path queries provide a useful mechanism for querying data
in many application domains. 
For example,
consider the knowledge base dataset
of the Linked Open Data (\lod) cloud.  
\lod\ is a community effort which aims to 
interlink the structural information available in various datasets
on the Web (such as Wikipedia, WordNet, and others), 
and make it available as a single \rdf\ graph.

\rpq s prove useful in querying such linked data
by providing a convenient declarative mechanism 
which can be used 
to answer queries without prior knowledge of 
the underlying data paths. 
% We illustrate this by the following example.

% example: RPQ query scenario
\begin{example} \label{EX LOD}
Consider the part of a \lod\ graph database
as presented in Fig.~\ref{fig:graph_eg}.
This represents information
the Gundam robot statue in Odaiba in Tokyo.
The data has been integrated from two datasets,
identified by the prefixes \textsf{en} and \textsf{jp},
standing for the English and Japanese Wikipedia,
respectfully.
The data entities between these two datasets are
interlinked by using OWL ontology terms.
Equivalent entities are connected
with \textsf{owl:sameAs} edges.
In this case,
the Japanese dataset contains richer spatial information
related to the statue than does the English dataset.

%Consider a data exploration scenario in which 
%a user wants to know in which country this Gundam statue is located.
%RPQs provide a convenient mechanism which can be used 
%to answer this question without prior knowledge of 
%exact underlying data paths and utilizing 
%the information from all linked datasets:
%\begin{center}
%\(Q =\,\,\)
%	\textsf{d1:Gundam (:sameAs*/:isLocatedIn)+/:sameAs* ?place}
%\end{center}
%Above, $Q$ computes the \textsf{:isLocatedIn} closure
%which originates from \textsf{en:Gundam} 
%at the same time resolving all OWL \textsf{:sameAs}
%equivalence classes (which requires a closure computation on its own).
%Note that since there is no direct connection from 
%\textsf{en:Gundam} to 

Say a user wants to know in which country
this Gundam statue is located.
Since there are no direct \textsf{:isLocatedIn} edges
outgoing from \textsf{en:Gundam}---%
as is often the case in linked data---%
the graph needs to be \emph{searched}.
During the search,
equivalent data entities need to be resolved 
by following \textsf{:sameAs} edges.
Likewise,
a spatial hierarchy needs to be computed by following 
\textsf{:isLocatedIn} edges.
This search can be defined
by the following \sparql\ query pattern:

\begin{prolog}[\sf]
% \(Q =\,\,\)
	\qquad\qquad\=\kill
	en:Gundam (:sameAs*/:isLocatedIn)+
	\plabel[Q gundam]{querynum}
	\+\\
		/:sameAs* ?place .
\end{prolog}

\noindent
\ref{Q gundam} computes the spatial hierarchy 
starting from node \textsf{en:Gundam},
using information from both interlinked datasets
to resolve equivalent entity closures.
\end{example}

\end{Sect}
%----------------------------------------------------------------------------%
\begin{Sect}{FA Plans}
\label{SEC/bg/auto}

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% generators and recognizers

% In general,
Regular expressions are a formal notation
for patterns that \emph{generate} strings---%
called \emph{words}---%
over an \emph{alphabet}.
The set of words
that a given regular expression can generate
is called its \emph{language}.

The dual to generation is \emph{recognition}.
\emph{Finite state automata} are the recognition
counterpart to regular expressions.
For any given regular expression,
a finite state automaton---%
abbreviated as \emph{finite automaton}---%
can be constructed
that will \emph{recognize}
% ---
% or \emph{classify}---%
the words over the alphabet
that belong to the expression's language.

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% finite automata (deterministic)

% Formally, a {\em deterministic finite automaton} \(A\)
% is defined as the tuple \tuple{Q, \Sigma, \delta, q_0, F}\
% for which
% 	\(Q\) is a finite set of states,
% 	\(\Sigma\) is a finite \emph{alphabet}
% 		(a set of symbols),
% 	\(q_0 \in Q\) is the \emph{start state},
% 	\(F\subseteq Q\) are the {\em final} (or \emph{accepting}) {\em states},
% 		and
% 	\(\delta\) is the \emph{transition function}
% 		which maps pairs of states and symbols to states.
% The \emph{size} of automaton \(A\)
% is measured as its number of states,
% \(|Q|\).

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% a run of an automata / a language of automata

% A {\em run} of automaton \(A\)
% on an input word \(w = w_1 \ldots w_n\)
% is the sequence of states \(q_0 \ldots q_n \in Q\)
% such that \(q_0\) is \(A\)'s start state
% and \(q_i = \delta(q_{i-1}, w_i)\),
% for \(0 < i \leq n\).
% The word \(w\) is said to be \emph{accepted}
% by automaton \(A\) if the run \(A(w)\) finishes in an accepting state,
% \(q_n \in F\).
% (Word \(w\) is said to be {\em rejected}, otherwise.)
% The set of all words (finitely composable over \(\Sigma\))
% recognized by automaton \(A\)
% defines the {\em language} that is
% recognized by automaton \(A\).

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% non-deterministic FAs 

% {\em Non-deterministic finite automata} (NFAs)
% generalize deterministic finite automata (DFAs)
% by allowing an FA to be in multiple states simultaneously
% during runs.
% We redefine 
% \(\delta\) to map 
% from pairs of states and symbols to {\em sets} of states.
% A run of \(A\) on \(w\) is then redefined as
% the sequence of sets of states
% \(Q_0 \ldots Q_n \subseteq Q\)
% such that \(Q_0 = \{q_0\}\) where \(q_0\) is \(A\)'s start state
% and \(Q_i = \bigcup_{q_{i-1}\in Q_{i-1}}\delta(q_{i-1}, w_i)\),
% for \(0 < i \leq n\).
% The word \(w\) is \emph{accepted} by \(A\)
% if there is a final state within \(Q_n\),
% \(F\cap Q_n \ne \emptyset\).

% It is known that NFAs do not increase {\em expressiveness} over DFAs;
% for any language recognized by an NFA,
% there exists a DFA that also recognizes it.
% However,
% NFAs are more {\em compact};
% there are languages for which all corresponding DFAs
% are exponentially larger in size than an NFA for the language.

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% automaton construction

Thus,
an \fa\ \(A\) can be constructed to recognize the language
of a given regular expression \(r\).
One can construct one such \fa\
by traversing the parse tree of \(r\) bottom up,
and combining the automata
that recognize sub-expressions of \(r\)
into a composite automaton via
	union,
	concatenation,
		and
	closure
of the sub-automata as is appropriate.

% example: conversion pp -> NFA
\begin{example} \label{EX NFA}
Recall query \ref{Q gundam} from Ex.~\ref{EX LOD}.
As shown in Fig.~\ref{fig:eg_parse_tree_nfa},
an automaton construction for this query is
a two-step procedure.
First,
traversing the parse-tree of \(r\) bottom up,
the \enfa\ is built up,
by the base case
and the inductive rules.
Second,
the resulting \enfa\ is then
\emph{minimized} to an \nfa, 
which typically has smaller size,
and hence,
is more efficient to process.
\end{example}

% (figure: example NFA and its simplification)
\begin{figure}
	\centering
	\includegraphics[width=.48\textwidth]{eg_parse_tree_nfa.tikz}
	\caption{%
		An $\epsilon$-NFA and corres.~reduced NFA for \ref{Q gundam}.
	}
	\label{fig:eg_parse_tree_nfa}
\end{figure}
% (end)

% evaluation in G+
The first algorithm to use automata 
to evaluate regular expressions on graphs 
was presented in \cite{mendelzon1995finding} 
as a part of an implementation
of the \textbf{G+} query language.
%
Given a graph database $G=(N,E)$ and a query $Q=(s,L(r),t)$ 
in which $s$ and $t$ are nodes in $G$,
the algorithm proceeds as follows. 
The expression $r$ is converted into a finite automaton $A_Q$ 
by using the bottom up traversal of parse tree of $r$,
as discussed. 
%
Then, the graph database $G$ is converted to finite automaton $A_G$ 
with graph nodes becoming automaton states and graph edges becoming transitions. 
Node $x$ is assigned to be the initial state,
and $y$ is assigned to be the accepting state in $A_G$. 

Then,
given $A_G$ and $A_Q$,
a product automaton $P = A_G \times A_Q$ is constructed. 
%
$P$ is then tested for non-emptiness, 
which checks
whether any accepting state can be reached from the initial state. 
If the language defined by $P$ is not empty, 
then the answer for the reachability query $(s,L(r),t)$ on graph $G$ is ``yes''; 
i.e., there exists a path between $s$ and $t$ in $G$ that conforms to $r$. 
%
This idea of employing a product automaton
for \rpq\ evaluation
over graphs has been used in
\cite{%
	zauner2010rpl,%
	perez2010nsparql,%
	mendelzon1995finding,%
	kochut2007sparqler,%
	koschmieder2012regular,%
	consens1995constant
}.

% example: product automaton evaluation
\begin{example} \label{EX Prod-NFA}
Given query \ref{Q gundam} and the database $G$
from Ex.~\ref{EX LOD},
the corresponding product automaton $P = A_G \times A_Q$ is shown
in Fig.~\ref{fig:eg_product_nfa}.
$P$ is a representation of the \emph{search space}
that needs to be explored
to answer \ref{Q gundam}.
$P$ can be explored using any search strategy---%
e.g., breadth-first search---%
starting from the initial state
$\tuple{\text{\textsf{en:Gundam}},q_0}$.
All reachable accepting states (shown in bold) are
the answers to \ref{Q gundam}.

\end{example}

% (figure: example of product automaton construction/evaluation)
\begin{figure}
    \centering
    %\input{eg_prod_automaton.tikz}
    %\includegraphics[width=0.45\textwidth]{eg_prod_automaton.png}
    \includegraphics[width=0.45\textwidth]{eg_prod_automaton.tikz}
    \caption{Example product construction of automata.}
    \label{fig:eg_product_nfa}
\end{figure}
% (end)

% Based on this algorithm, we observe that a problem of answering an
% RPQ breaks down into two subproblems. First, a path \emph{recognition}
% tests whether a given path-induced label conforms to a given regular
% expression. And second, a path \emph{search}, finds all pairs of
% nodes in a given graph such that a path between them is recognized
% by a given regular expression. The evaluation strategies that
% construct a product automaton to answer an RPQ effectively do not
% make a distinction between \emph{search} and \emph{recognition}
% sub-problems. The main drawback of these approaches is that for
% each given query, the graph database needs to be translated into
% an automaton with subsequent product computation and non-emptiness
% verification. This process is not feasible for large graphs that
% do not fit into primary memory.

% To address this problem, path search and expression recognition are
% separated in the approach by Kochut et al.\cite{kochut2007sparqler},
% thus eliminating the need of conversion of the graph database into
% an automaton. In this algorithm, path recognition is performed for
% every added vertex during the breadth-first search. Thus, during
% the execution all paths are stored (or recomputed) and checked
% against the automaton. Both of these operations are very costly on
% large graphs. This problem is addressed by Koschmieder et
% al.\cite{koschmieder2012regular} by introducing the idea of advancing
% in both the graph and the automaton, and thus performing search and
% recognition simultaneously. In this case, no paths need to be stored
% or verified against the expression. In fact, graph nodes marked
% with accepting states during the search are correct query solutions
% (i.e., a path between a node marked accepting state and a node
% marked initial state conforms to a regular expression specified in
% a query).

%<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<%
\end{Sect}
%----------------------------------------------------------------------------%
\begin{Sect}{{\large\(\bm\alpha\)}-RA Plans}
\label{SEC/bg/DP-based}

% (figure: example parse tree and corresponding evaluation via RA tree)
\begin{figure}
	\centering
	\includegraphics[width=.4\textwidth]{eg_parse_ra_trees.tikz}
	% \caption{A parse tree and $\alpha$-RA tree for query $Q$.}
	\caption{A parse tree and $\alpha$-RA tree for query \ref{Q gundam}.}
	\label{fig:eg_parse_ra_trees}
\end{figure}
% (end)

An alternative approach
% This group of algorithms
is to use
the \(\alpha\)-extended relational algebra
(\ara)
to produce evaluation plans for \rpq s.
%
The \(\alpha\) operator computes
the transitive closure of a relation.
%
Let the graph database be represented as
a relation of triples $G(s,p,o)$.
Let $T = \pi_{1,3}G$;
thus $T$ consists of
pairs of nodes \tuple{s,o} such that the pair is
connected by a directed edge im the graph.
%
Then
$\alpha$ applied to \(T\) computes the \emph{least fixpoint}
of the following operation:

\begin{prolog}
	$T^+ = T \cup \pi_{1,3} (T^+ \bowtie_{{T^+}.o=T.s} T)$
	\plabel[EQ lfp]{eqnum}%
\end{prolog}

\noindent
Thus,
$\alpha(T)$ results in all pairs of nodes
such that,
for the nodes of each pair,
there \emph{exists} a path between them in the graph (denoted by) $G$.
% the determination of all paths in the graph. NO!!!
If we were to evaluate the fixpoint by a semi-na\"ive evaluation,
each iteration of evaluation
is over paths of length one greater than of the previous iteration.
The process stops when no new pairs are added;
i.e., the fixpoint has been reached.

Given the SPJRU (select-project-join-rename-union)
relational algebra extended with the $\alpha$ operator, 
one can evaluate the \rpq\ $Q=(x,L(r),y)$
over graph $G=(N,E)$
by the algorithm proposed
in \cite{losemann2012complexity}.
%Recently, Losemann et al.\cite{losemann2012complexity} 
%presented an RPQ evaluation algorithm that follows 
%a dynamic programming approach. 
%%
%Let $G=(N,E)$ be a graph database and $Q=(x,L(r),y)$ be a regular path query. 
This traverses the syntax tree of expression $r$ bottom-up. 
Let $s$ be the sub-expression of $r$
represented by a given node in a parse tree. 
% ??? -parke
% Then,
% for each node in the syntax tree which is associated with sub-expression $s$, 
%
The binary relation $R_s \subseteq N \times N$ is computed
so that node pair $(u,v) \in R_s$ \emph{iff}
there exists a path from $u$ to $v$ in $G$ that matches $s$.

The manner in which the relations are joined going bottom-up 
in a parse tree
depends upon the type of the node. 
The cases are as follows:

\begin{enumerate}
\item If $s$ is a $\Sigma$-symbol,
	then $R_s := \{(u,v) | (u,s,v) \in E \}$.

\item If $s=\epsilon$,
	then  $R_s := \{(u,u) | u \in N \}$.

\item If $s_1$ and $s_2$ are sub-expressions and $s = s_1 | s_2$,
	then $R_s = R_{s1} \cup R_{s2}$.

\item If $s_1$ and $s_2$ are sub-expressions and $s = s_1 \cdot s_2$,
	then $R_s = \pi_{1,3}(R_{s1} \bowtie_{R_{s1}.2 = R_{s2}.1} R_{s2}$.
% 	\footnote{%
% 		``$\bowtie_{R_{s1}.2 = R_{s2}.1}$'' denotes
% 		the ternary relation obtained by joining on $R_{s1}$ and $R_{s2}$
% 		by pairing tuples that agree on the right column of $R_{s1}$
% 		and the left column of $R_{s2}$.
% 		``$\pi_{1,3}$'' denotes the projection of these triples
% 		onto the leftmost and rightmost column.
% 	}

\item If $s=s_1^*$,
	then $R_s$ is the reflexive and transitive closure
	of $R_{s1}$, or $R_s = \alpha(R_{s1}) \cup R_{s1}$.

\item If $s=s_1^+$,
	then $R_s$ is the transitive closure of $R_{s1}$, or $R_s = \alpha(R_{s1})$.

\end{enumerate}

\noindent
(Correctness of this algorithm is established
in \cite{losemann2012complexity}).

% The correctness of this algorithm can be proved by 
% performing a structural induction and showing that 
% the following invariant holds for every relation $R_s$ that is calculated: 
% For each sub-expression $s$ of $r$, 
% we have $(u,v) \in R_s \Longleftrightarrow \exists$ path $p$ 
% in graph $G$ from $u$ to $v$ such that 
% its induced label $\lambda(p)$ belongs to language $L(s)$. 

% example: alpha-RA tree : Example 4
\begin{example}
Given query \ref{Q gundam} and the database $G$
from Ex.~\ref{EX LOD},
the corresponding \ara\ tree 
is shown in Fig.~\ref{fig:eg_parse_ra_trees}. 
\end{example}

%% (figure: example of Losemann et al.)
%\begin{figure}
%    \centering
%    \includegraphics[width=0.5\textwidth]{dp_eg.png}
%    \caption{Example run of an algorithm proposed by Losemann et al.}
%    \label{fig:dp_eg}
%\end{figure}
%% (end)

% Discussion
%The main advantage of this method is that it reduces the problem of answering a regular path query on graph to a bottom-up evaluation approach which utilizes algebraic operations on relations. This allows for tree-like compositions of operators that specify an evaluation \emph{plan} for a given RPQ. 

%In fact, similarity of these RPQ evaluation plans to plans defined by relational algebra, 

The $\alpha$-RA-based \rpq\ evaluation can be directly
implemented in most relational databases 
and relational triple-stores. 
In \cite{DBLP:conf/amw/YakovetsGG13},
% Yakovets et al.
we proposed a method that translates \rpq s
as defined by \sparql\ property paths
into recursive \sql. 
A similar approach was used by Dey et al.~
\cite{dey2013implementing} 
in the context of the evaluation
of provenance-aware \rpq s
by a relational engine.

%<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<%
\end{Sect}
%----------------------------------------------------------------------------%
% comparing plan space of FA and alpha-RA evaluation methods
\begin{Sect}{Comparing Plan Spaces}
\label{SEC/bg/plan_space}

% (figure: ...)
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{claim_img.tikz}
    \caption{Example plans.}
    \label{fig:claim_img}
\end{figure}
% (end)

The \fa\ and \ara\ approaches 
each entail a \emph{plan space};
that is,
the plans collectively an approach produces
over all possible property-path queries.
Let \planspace[\fa]\ and \planspace[\ara]\ 
denote the plan spaces for \fa\ and \ara, respectively.
To understand how the approaches are related---%
for instance, whether one approach subsumes the other,
or whether they are incomparable---%
we consider these plan spaces.
The Venn diagram of how they are related is shown
in Fig.~\ref{fig:claim_img}c.%
\footnote{%
	The diagram's claim that the plan space of waveguide plans,
	\planspace[\wgp], properly subsumes
	both \planspace[\fa]\ and \planspace[\ara]\ 
	is taken up in \S\ref{sec:WGP space}.
}

\begin{claim} \label{CLAIM incomparable}
\planspace[\fa]\ and \planspace[\ara]\ 
are \emph{incomparable}
(\(\planspace[\fa] - \planspace[\ara] \neq \emptyset\)
and
\(\planspace[\ara] - \planspace[\fa] \neq \emptyset\)),
but \emph{overlap}
(\(\planspace[\fa]\cap\planspace[\ara] \neq \emptyset\)).
\end{claim}

Of course,
we are taking liberties;
the place spaces should be over the same \emph{domain} of plans.
As we have presented things,
however,
they are not;
we have presented \fa\ plans as automata
and \ara\ plans as algebraic trees.
%
To prove formally the claim in Fig.~\ref{fig:claim_img}c,
we would need to establish an isomorphism
between \fa\ and \ara\ plans,
or have a canonical form for plans
to which each plan type could be mapped.
This can be done.
The formalism for waveguide plans
we will present in \S\ref{sec:eval}
would suffice for this mapping.
\datalog,
or the \emph{relational algebra} extended by \emph{while loops}
(established to be expressively equivalent to \datalog)
\cite{abiteboul1995foundations},
would provide an even more universal domain that would suffice.

This is beyond the scope of what we can do here.
Still,
we easily can establish informally that these spaces are distinct.
Consider the following \emph{generic} property-path query pattern:

\begin{prolog}[\sf]
	?x (a/b)+ ?y .
	\plabel[Q AB+]{querynum}%
\end{prolog}

\noindent
We shall be using \ref{Q AB+} as a prevalent example.
Here, ``\textsf{a}'' and ``\textsf{b}'' are stand-ins for labels.
It matches node-pairs that are connected by some path labeled
\textsf{ab}, \textsf{abab}, or \textsf{ababab},
and so forth.
This is a quite simple property-path query,
but one that already demonstrates the complexities of planning.

The \fa\ plan in Fig.~\ref{fig:claim_img}a
would be in \planspace[\fa]\ for \ref{Q AB+}.
There is no \ara\ plan that could be equivalent to it,
however;
none would ever evaluate \textsf{aba}, \textsf{ababa}, and so forth
as state \state{q}[1]\ does in the \fa\ plan.
\ara\ plans cannot compute transitive closure in a \emph{pipelined} fashion
as the \fa\ plan is doing;
the \(\alpha\) operator acts over an entire relation.

The \ara\ plan in Fig.~\ref{fig:claim_img}b
would be in \planspace[\ara]\ for \ref{Q AB+}.
There is no \fa\ plan that could be equivalent to it,
however;
no state transition in its automata can represent the ``join''
with \textsf{ab}.
\fa\ plans do not encompass \emph{views},
materialized parts of the query that can be reused,
while the \ara\ plan does by effectively materializing \textsf{ab}
to join repeatedly on it.

Meanwhile,
there are many plans in common between \fa\ and \ara:
for any query that is restricted to transitive closure
over single labels,
for example,
will result in common \fa\ and \ara\ plans.

% We define an \emph{evaluation plan} for $Q$
% as a sequence of operations the algorithm should follow
% in order to produce an answer to $Q$.
% Given an RPQ $Q$,
% there are many plans the algorithm may use.
% All such plans are equivalent in terms of their final output,
% but vary in their cost, or the amount of time the algorithm needs to run.
% Then, \emph{plan space}, is a set of all evaluation plans 
% that the algorithm may follow to answer a given query.
% %Here, we consider a high-level specification of plans
% %(e.g. in which order the operations are performed)
% %but not low-level physical plans (e.g. which join method is used).

% In $\alpha$-RA-based search a high-level evaluation plan 
% is an $\alpha$-algebra operator tree.
% An initial tree is produced by a by bottom-up traversal 
% of a parse tree of $Q$. 
% Then, this tree can be transformed by the application
% of a number of rewrites based on
% relational algebra equivalences
% (such as join commutativity, selection pushdown, etc.).
% The set of all such equivalent $\alpha$-RA trees
% comprises an $\alpha$-RA plan space
% $\mathcal{P}_{\alpha\text{-RA}}$.

% On the other hand, in FA-based methods,
% % need to emphasize here
% the search space explored by the evaluation algorithm depends
% on a finite automaton constructed from $Q$.
% An initial automaton is obtained directly by 
% following standard construction procedure based on 
% regular expression $r$ in $Q$.
% Then, this automaton can be transformed
% by employing automata minimization procedures.
% A set of all automata that recognize $r$ comprises an 
% FA plan space $\mathcal{P}_{\text{FA}}$.

% % claim: a-RA not subset of FA
% \vspace{2mm}
% \noindent
% \textbf{Claim 1.}
% $\mathcal{P}_{\text{FA}} \not\subset \mathcal{P}_{\alpha\text{-RA}}$
% \\ 
% \noindent
% \textbf{Proof sketch:} Proceed with proof by example. 
% We need to find at least one plan $P$ such that $P \in \mathcal{P}_{\text{FA}}$
% and $P \not\in \mathcal{P}_{\alpha\text{-RA}}$. 
% Consider an evaluation plan for query $Q = (x, (ab)+, y)$.
% %
% % claim: FA not subset of a-RA
% \vspace{2mm}
% \noindent
% \textbf{Claim 2.}
% $\mathcal{P}_{\alpha\text{-RA}} \not\subset \mathcal{P}_{\text{FA}}$
% \\ 
% \noindent
% \textbf{Proof sketch:} Consider the same query $Q$ as in Claim 1. 

\end{Sect}
%----------------------------------------------------------------------------%
\end{Sect}


==> conc.tex <==
%!TEX root = paper.tex

%============================================================================%
\begin{Sect}{Next Steps \& Conclusions} \label{sec:conc}

Waveguide plans model a rich space of plans for path queries
which encompass powerful optimization techniques.
Next steps in this endeavor are as follows.

\begin{enumerate}
\item 
	\emph{Benchmark}
	\waveguide\ against
	current, prevalent \sparql\ engines
	that support property path queries
	(e.g., \jenaTDB, \virtuoso, and \allegrograph).

\item 
	\emph{Build}
	a full-fledged \emph{cost-based query optimizer}
	for \sparql\ 1.1 for property paths (\rpq s).

	\begin{enumerate}
	\item 
		\emph{Define}
		``\wgp'' systematically to define formally
		the \emph{space} of \wgp s for a given query.

	\item 
		\emph{Devise}
		a concrete \emph{cost model} for \wgp s.

	\item 
		\emph{Determine}
		an array of \emph{statistics}
		(e.g., 1-gram and 2-gram label frequencies)
		that can be computed efficiently offline
		that can be used in conjunction with the cost model.

	\item 
		\emph{Design}
		an enumeration algorithm to walk dynamically the space of \wgp s
		to find the \wgp\ with least estimated cost.

	\end{enumerate}

\item 
	\emph{Extend}
	the \emph{query optimizer} to handle
	queries queries with multiple property-paths
	(equivalent to \emph{conjunctive} regular path queries).

\end{enumerate}

Just as new data models necessitate new query languages,
these new query languages necessitate new approaches
if we are to evaluate their queries efficiently and effectively.
The rise of graph databases has necessitated
new, powerful query languages
so that we can make use of them.
But we are only beginning
to uderstand how we can deal effectively
with these types of queries.

In this work,
we have devised a rich domain of evaluation plans 
for property-path type queries in \sparql,
and have shown it extends significantly over the state of the art.
%
We have demonstrated that choice of plan can make
orders of magnitude difference in performance.
We have illustrated the cost factors behind these plans's performance
and the types of optimizations that can be achieved.
%
We have shown which plans are effective
depends on the underlying graph database,
which means a cost-based means of choosing plans is required.
The rise of graph data is well underway.
And as we learned in the past to do the ``impossible''
for relational data, for semi-structured, for unstructured search,
we too will meet this challenge.

% In initial benchmarking against leading \sparql\ systems,
% we are able to match the query ``plans'' via \wgp s
% that the other systems essentially devise.
% With these \wgp s,
% \waveguide\ usually matches or exceeds the others' performance.
% (This is due to additional optimizations in \waveguide\
% and its evaluation approach.)
% In many cases,
% however,
% we are able to find alternative \wgp s
% that outperform the other systems heavily,
% as \wgp s offer a much richer plan space
% than is effectively covered by them.

% With \waveguide,
% we intend to provide viable cost-based query optimization
% for \rdf\ and graph databases
% analogous to the state of the art
% for relational database systems.

%----------------------------------------------------------------------------%
\end{Sect}


==> cost.tex <==
%!TEX root = paper.tex
%============================================================================%
\begin{Sect}{Plan Costs} 
\label{sec:CoP}

For a given query,
of course,
there may be many ways to guide the search.
% In this section
We summarize 
	a \emph{cost framework} for \waveguide\ search,
	\emph{search cost factors} that can magnify the cost
	(properties of the graph
	and of resulting pre-paths computed during evaluation),
		and
	\emph{optimization methods}
	that are enabled by \wgp s
	which address the search factors, in turn.

%----------------------------------------------------------------------------%
\begin{Sect}{Cost Framework} \label{sec:cost_framework}
%
Recall the three steps
in Fig.~\ref{fig:direct_search_algo}
of the search iteration:
	\crank,
	\reduce,
		and
	\union. 
%
% The total cost is the sum of costs of these operations
% over the iterations:
% 
% $$
% cost = 	cost(\text{\textsf{crank}}) + 
% 		cost(\text{\textsf{reduce}}) + 
% 		cost(\text{\textsf{union}})
% $$
%
Assume that the search completes in \(n\) iterations.
The cost of \crank, \cost[\crank], corresponds 
to the total number of \emph{edge walks} performed.
% during the search
This \emph{search size} is the sum of sizes of the deltas.
%
The cost of \reduce, \cost[\reduce],
has two components: 
	duplicate removal
		within a delta
			and
		for the delta against the search cache.
Cost of removal against the delta is often cheaper,
since in can be implemented in-memory,
while checking against the cache,
due to its larger size, 
might require
implementation on secondary storage, 
therefore increasing its cost.

% Finally,
The cost of \union, \cost[\reduce],
is associated
with search cache maintenance procedures (e.g., indexing),
and depends on the size of the search cache.

\begin{enumerate}
\item
	\(\displaystyle
		\cost[\crank] = \sum_{i=0}^{n} f_1(|\Delta_i|)
	\)

\item
	\(\displaystyle
		\cost[\reduce] = \sum_{i=0}^{n}%
			\left(%
				f_2(|\Delta_i|) + f_3(|C_i|)%
			\right)
	\)

\item
	\(\displaystyle
		\cost[\union] = \sum_{i=0}^{n} f_4(|C_i|)
	\)

\end{enumerate}

\noindent
The cost functions \(f_{1-4}\) above
are monotone over their parameters;
these simply abstract the actual costs
as based upon the underlying implementation
of \waveguide's data structures and algorithms.

\end{Sect}
%----------------------------------------------------------------------------%
\begin{Sect}{Search Cost Factors} \label{sec:factors}
%
Properties of the graph and of the \wgp\ chosen---%
so the guided search as performed
in terms of the pre-paths that are computed by the search---%
will determine the evaluation cost.

%\vspace*{0.25ex} this wasn't doing anything... fix from: http://texhacks.blogspot.ca/2010/12/vspace-is-broken.html
\Vspace{3pt}
\noindent
\emph{Search Cardinalities}.
The \emph{wavefront}, or \emph{wavefronts},
that we choose---%
as dictated by the wavefronts of the \wgp---%
for the search
determines the intermediate results
(pairs of nodes connected by valid pre-paths)
that we collect each iteration.
Just as with different join orders in relational query evaluation,
different wavefronts will result in different intermediate delta sizes.
These intermediate cardinalities can vary widely from plan to plan.

%\vspace*{0.25ex}
\Vspace{3pt}
\noindent
\emph{Solution Redundancy}. 
After much deliberation in the research community, 
the W3C has adopted a \emph{non-counting} semantics
for \sparql\ property-path queries. 
Each node pair appears at most once in the answer, 
even if there are several paths between the node pair
satisfying the given regular expression. 

Answer-path redundancy arises from two sources.
First,
in dense graphs,
solutions are re-discovered
by following conforming, yet different paths.
Second,
nodes are revisited by following cycles in the graph.  
%
Thus,
the same answer pair
may be discovered repeatedly during evaluation.
%
It is critical to detect such duplicate solutions early
in order to keep the search size and search cache small.

% This leads to \emph{solution redundancy};
% i.e., generation of unnecessary duplicate answer node pairs 
% during the query evaluation process.

% We discuss which properties of the graph database contribute
% to the cost of \waveguide\ search.
% As we've shown, 
% one of the defining search cost factors is search size, 
% which is the sum of all edge walks during the cranks.
% Then, 
% given a query expression, 
% it is useful to look 
% at the \emph{cardinality} of its edge labels in the graph database.
% Labels with \emph{low} cardinality may indicate 
% query \emph{chokepoints},
% or sub-expressions that constrain 
% the flow of the wavefront the most.
% These are useful in designing 
% a plan with the smallest estimated search size.

%\vspace*{0.25ex}
\Vspace{3pt}
\noindent
\emph{Sub-path Redundancy}.
In \emph{solution redundancy},
an answer pair could have multiple paths justifying it.
Likewise,
the paths justifying multiple answer pairs
may \emph{share} significant segments (\emph{sub-paths}) in common.

This arises, for instance,
in dense graphs and with hierarchical structures
(e.g., \emph{isA} and \emph{locatedIn} edge labels).
Consider a query ``\textsf{?p :locatedIn+ Canada}''.
Every person located in the neighborhood of the Annex
in the city of Toronto qualifies,
since the Annex is located in Toronto
which is located in Ontario
which is located in Canada.
The sub-path ``\textsf{Annex :locatedIn+ Canada}''
is shared by the answer path for each Annex resident.

Because we keep only node-pairs (plus state) in the search deltas,
and not explicitly the paths themselves,%
\footnote{%
	Note this design choice in our evaluation strategy
	is critical for good performance
	due to solution redundancy!
}
we may walk these sub-paths many times,
recomputing ``\textsf{Annex :locatedIn+ Canada}''
for each Annex resident.

% figure: search cost factors
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{search_factors.tikz}
	\caption{Types of search cost factors.}
	\label{fig:search_factors}
\end{figure}

% conforming sub-paths are often \emph{shared} among candidate solutions.
% In this situation,
% during the search, 
% these paths are effectively re-computed 
% over and over again
% for each of the candidate solutions.

% In order to avoid this wasteful re-computation and 
% reduce both search size and search cache, 
% it is beneficial to compute these sub-paths 
% in a separate sub-wavefront, 
% the results of which are then joined 
% with the main wavefront to produce the final solutions.

\end{Sect}
%----------------------------------------------------------------------------%
\begin{Sect}{Plan Optimizations} \label{sec:methods}
%
% Our goal, 
% given a graph database and a SPARQL property path query,
% is to design a \waveguide\ query plan automaton 
% such that it guides 
% an \emph{efficient} search that fits 
% given time and space constraints.
% Here, 
We consider \wgp-optimization methods
in relation to the search cost factors above.
% that aim to minimize the total estimated cost of evaluation.

%\vspace*{0.25ex}
\Vspace{3pt}
\noindent
\emph{Choice of Wavefronts}.
The direction in which we follow edges,
and where we start in the graph,
with respect to the regular expression
will result in different \emph{search cardinalities}.
Our choice of automata in the \wgp\ dictates the wavefront(s).
%
For example, consider query $Q=(x,(abc),y)$ and a fragment of 
a graph shown in Fig.~\ref{fig:search_factors}a.
Since labels $a$, $b$ and $c$ have different cardinalities,
different wavefronts will have different search size.
Consider two plans $P_1$ and $P_2$ that evaluate $Q$
shown in Fig.~\ref{fig:opt_methods}.
$P_1$ has a single wavefront that 
explores the graph starting from $a$, 
appending $b$ and then $c$.
On the other hand, $P_2$ has a wavefront that 
starts from the low cardinality label $b$,
appends $c$ and then prepends $a$.
Observe that, in this scenario, 
$P_2$ results in fewer edge walks than $P_1$.

To reduce overall search size,
we need to choose wavefronts
that result in fewer edge walks.
Wavefronts can be costed to estimate their search sizes
based on statistics about the graph,
such as $1$-gram and $2$-gram label frequencies.
(Such graph statistics can be computed offline for this purpose.)

% figure: search cost factors 1
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{opt_methods.tikz}
	\caption{Choosing the wavefronts.}
	\label{fig:opt_methods}
\end{figure}

% % multiple wavefronts at chokepoints and SIP
% Recall that query chokepoints may be a helpful graph statistic 
% in designing an efficient query plan.
% QPA, unlike NFA-based plans,
% are able to guide multiple wavefronts from 
% different starting points and directions.
% Then, 
% a possible \emph{greedy} strategy is
% to design a plan such that wavefronts originate from
% one or more chokepoints and expand in the opposite directions.
% When these wavefronts compute 
% their respective regular sub-expressions, 
% they are joined to produce the final result.
% This strategy ensures the smallest initial search size,
% which, 
% in optimistic scenarios, 
% results in the search size reduction 
% throughout the whole process of the search.
% Moreover, 
% those opposite-direction wavefronts 
% that share the starting point
% introduce additional optimization opportunities 
% similar to sideways information passing (SIP, \cite{}).  
% In this scenario, SIP-like run-time pruning 
% works as follows. 
% Every \textsf{crank} operation, 
% each shared starting seed is checked 
% if it has expanded by both outgoing wavefronts.
% If the seed fails to expand by at least one wavefront,
% it is removed from the delta by 
% subsequent \textsf{reduce} operation
% to prevent further expansion by the opposite wavefront. 

%\vspace*{0.25ex}
\Vspace{3pt}
% reduce at delta and reduce at cache
\noindent
\emph{Reduce}.
\waveguide's evaluation strategy is designed to counter solution redundancy. 
% Specifically, we consider \emph{pre}-solution and
% \emph{post}-solution redundancy.
As shown in Fig.~\ref{fig:search_factors}b,
we consider several types of redundant solutions
based on a path which was followed to obtain
each solution.
Path A is a shortest path.
Paths B and B$'$ are of the same length,
but go through different nodes.
Finally, path C$'$ shares 
some nodes with path C, 
but it is longer due to a cycle.

In \waveguide, redundancy of \emph{candidate} solutions
is addressed by removal of duplicates
against both cache (\textsf{cache})
and delta (\textsf{delta})
by the \reduce\ operation.
%
Assuming BFS search strategy,
duplicate solutions obtained by following paths 
of the same length (B, B$'$) are removed within a delta.
On the other hand, 
duplicates obtained by following paths of 
different lengths (A, B) are removed 
when delta is compared against a cache.
This also includes paths with cycles such as C and C$'$
as they also have different length.

As a further optimization,
once a solution seed-target pair has been discovered,
\emph{first-path pruning} (\textsf{fpp})
removes the \emph{seed} from further expansion
by the search wavefronts.
In our example, 
once path A has been discovered and solution $(x,y)$ 
has been obtained, all longer paths (B, B$'$, C, C$'$)
are never even materialized.

%\vspace*{0.25ex}
\Vspace{3pt}
% threading sub-wavefronts
\noindent
\emph{Threading}.
To counter \emph{sub-path redundancy}
requires us to decompose a query into sub-queries.
We call this decomposition \emph{threading},
and our \wgp s accommodate this.

Consider query $Q = (x, (r_1/r_s/r_2), y)$
where
sub-path $r_s$ is shared among many 
solutions as shown in Fig.~\ref{fig:search_factors}c.
This query can be threaded as follows.
First, pre-path $r_1$ is computed by wavefront $W_{r_1}$.
Then, the portion of the regular expression
that will result in sub-paths that will be shared by many answer paths
can be computed by a separate wavefront $W_{r_s}$.
Here, $W_{r_1}$ seeds wavefront $W_{r_s}$
which computes a shared path for each of the 
partial solutions 
produced by $W_{r_1}$.
Finally, the complete path is pieced together by wavefront $W$.

Such sub-path sharing can be predicted by graph statistics
to indicate when sub-queries should be considered.

% figure: search cost factors 2
\begin{figure}
	\centering
	\includegraphics[width=0.6\linewidth]{opt_methods_2.tikz}
	\caption{Threading a shared sub-path.}
	\label{fig:opt_methods_2}
\end{figure}

% We deal with sub-path sharing by introducing 
% a new type of state
% \emph{threaded} states in query plan automata.
% When the search reaches a threaded state,
% the computation is \emph{restarted}
% by using intermediate \dots

%\vspace*{0.25ex}
\Vspace{3pt}
% partial materialization
\noindent
\emph{Partial Caching}.
Delta results are cached during evaluation
as we need to check against the cache for redundantly computed pairs.
For large intermediate cardinalities,
this can be a significant cost.
However,
some of this cost can be negated.
In particular,
not every state in the \wgp's automata
needs to have its node-pairs cached.
Caching is only needed when \emph{unbounded} 
redundancy is possible,
due to cycles in the wavefront automata or in the graph.
States without cycles need not be cached.

%\vspace*{0.25ex}
\Vspace{3pt}
% loop caching
\noindent
\emph{Loop Caching}.
Transitions over views in wavefront automata allows
us to cache and re-use some of
the intermediate node pairs
we encounter during the search.
Such named result sets are useful
in reducing unnecessary re-computation
by employing an optimization we call
\emph{loop caching}.

In transitive query $Q = (x, (r)+, y)$,
the expression $r$ is evaluated 
repeatedly until no new solutions are found.
Loop caching rewrites 
an evaluation plan such that the base $r$
is cached either fully or partially 
to speed up the transitive evaluation of $(r)+$. 

Consider three plans $P_{nc}$, $P_{pc}$ and $P_{fc}$ 
for query $Q = (x, (abc)+, y)$
shown in Fig.~\ref{fig:loop_caching}.
Plan $P_{nc}$ has no loop caching
as it evaluates full expression $(abc)$
in a loop.
Plan $P_{pc}$ uses a separate wavefront to 
evaluate $(bc)$ first, 
then these results are used
in a loop to evaluate transitive $(abc)+$.
Finally, plan $P_{fc}$ caches full
base expression $(abc)$, which is then used
in evaluation of a transitive expression.


% figure: search cost factors
\begin{figure}
	\centering
	\includegraphics[width=0.8\linewidth]{loop_caching.tikz}
	\caption{Types of loop caching.}
	\label{fig:loop_caching}
\end{figure}

% % partial materialization
% In \waveguide, 
% the intermediate search results
% are materialized in the search cache.
% This cache serves two main purposes.
% First, 
% it is used to in \textsf{crank} operation 
% to extend the wavefronts by using tuples
% from the cached \emph{views}.
% Second, \dots

%search cache $S$ is used 
%to keep the intermediate search results.

%Notice that \textsf{crank} operation 
%requires only the previous delta

%the factors 
%that contribute to the cost of the overall evaluation plan. 
%Then, we describe a number of techniques specific to \waveguide\ that deal 
%with these factors.

%\noindent \textbf{Search space.} 
%Total space explored by the search  
%is one of the defining factors of the cost of the query evaluation.

% process in order to answer a given query.
% Hence,
% it is important to design an automaton
% such that it guides an \emph{efficient} search
% that fits given time and space constraints.
%A good \qpa\ achieves a balance of
%	exploring a small search space,
%	re-using as much computation as possible
%	(by use of views),
%		and
%	having a simple controlling automaton.%
%\footnote{%
%	The cache contains tuples of the form \tuple{a,b,\state{s}}\
%	for which \state{s}\ is a state from the \qpa.
%	Two tuples \tuple{a,b,\state{r}}\ and \tuple{a,b,\state{s}}\
%	are different as they are from different states.
%	A \qpa\ with \emph{fewer} states
%	\emph{minimizes} this differentiation
%	and thus \emph{maximizes} ``duplication'';
%	i.e., the chance of discarding \tuple{a,b}\ 
%	when found again.
%}
%These three goals often cannot be independently obtained,
%which complicates plan construction.
%We demonstrate a simple cost-based \qpa\ generator
%ased on the \emph{cardinality} of graph labels.
%We focus on the labels with \emph{low} cardinality;
%i.e., \emph{rare} labels.
%Given a query expression,
%we can estimate its \emph{chokepoints},
%sub-expressions that constrain the flow of the wavefront the most.
%Based on these chokepoints,
%we design a \qpa\
%which would explore the smallest estimated search space.

\end{Sect}

\begin{Sect}{Cost Analysis}
\label{sec:cost_analysis}

In this section we analyze the cost of plan optimizations that are 
exclusive to \waveguide\ approach, 
such as threading and loop caching, 
with relation to the cost model 
presented in Section \ref{sec:cost_framework}.

\Vspace{3pt}
% threading sub-wavefronts
\noindent
\emph{Costs of threading}.  
Given a plan $P$ with a single wavefront which computes 
a regular expression of a form $r = r_1/r_s/r_2$,
threading rewrites it into a plan $P_t$ with three wavefronts 
$W_{r_1}$, $W_{r_s}$ and $W_{\text{join}}$
as described in Section \ref{sec:factors}.
Regardless of the split of $r$ into $r_1$, $r_s$ and $r_2$,
this optimization requires an additional cost of
an extra join in $W_{\text{join}}$.
If a shared sub-path $r_s$ is accurately identified,
then the total reduction of number of edge walks in $P_t$
is sufficiently large to offset the cost of the extra
join.

A useful graph metric in identifying the threading split is 
a \emph{multiplicity} ratio of an expression $r$ in graph $G$,
which is computed by analyzing the paths in $G$: 
$$
	\mathcal M(G,r) = \frac{|S_s|}{|S_o|},
$$
where $S_s$ and $S_o$ is a set of subjects and objects, respectively,
connected in $G$ with paths conforming to $r$.
Then, $\mathcal M(G,r)>1$, would indicate that, on average, there are many 
subjects connected to a single object in $G$, 
while $\mathcal M(G,r)<1$ would indicate that the opposite is true.
The greater $\mathcal M$ is, the more subjects are 
connected to the same object, 
and, hence, 
more subjects share a path which originates from this object.   

Another useful metric is an average length $\mathcal L(G,r_s)$ of a path
which conforms to $r_s$ in $G$. 
The longer the shared sub-path $r_s$ is,
the more potential savings in edge walks can be realized by 
threading split on $r_s$. 

Then,  
given $\mathcal M$ and $\mathcal L$ for sub-expressions of $r$
in $G$, the identification of an efficient threading split $r = r_1/r_s/r_2$ 
becomes an ($\mathcal M, \mathcal L$) maximization problem.

% TODO: missed opportunities to reduce..

%\begin{figure}[t]
%  \centering
%  \parbox{1.9in}{%
%  	\includegraphics[width=\linewidth]{loop_caching_lensing3.tikz}
%  	\caption{Lensing.}
%  	\label{fig:loop_caching_lensing}}
%  %\qquad
%  \begin{minipage}{1.3in}
%  	\includegraphics[width=\linewidth]{joins_serialization.tikz}
%  	\caption{Op.~order}
%  	\label{fig:joins_serialization}
%  \end{minipage}
%\end{figure}

\begin{figure}[t]
  \centering
  	\includegraphics[width=0.8\linewidth]{loop_caching_lensing3.tikz}
  	\caption{Lensing.}
  	\label{fig:loop_caching_lensing}
\end{figure}

%\begin{figure}
%  	\centering
%  	\includegraphics[width=\linewidth]{loop_caching_lensing2.tikz}
%  	\caption{Lensing.}
%  	\label{fig:loop_caching_lensing}
%\end{figure}
%
%\begin{figure}
%  	\centering
%  	\includegraphics[width=\linewidth]{joins_serialization.tikz}
%  	\caption{Serialization of ops.}
%  	\label{fig:joins_serialization}
%\end{figure}

\Vspace{3pt}
% threading sub-wavefronts
\noindent
\emph{Costs of loop caching}. 
Given a plan with a single wavefront which computes 
closure $(r)+$ of a regular expression $r$,
loop caching rewrites it into a plan in
which parts of $r$ are pre-computed, cached, and then
used in an iterative evaluation of a closure.
For example, consider the differences in evaluation of 
query $Q = (x, (abc)+, y)$ with
plans $P_{nc}$, $P_{pc}$ and $P_{fc}$
shown in Fig.~\ref{fig:loop_caching}.
$P_{nc}$ defines a single wavefront,
which, due to absence of transitions over views, 
can be executed pipelined. 
On the other hand,
$P_{pc}$ and $P_{fc}$ first compute $(bc)$ and $(abc)$,
respectively,
in separate wavefronts, the results of which
are used in a wavefront which computes the final closure.
Note that due to shorter cycles in wavefront automata in
cached plans $P_{pc}$ and $P_{fc}$,
the total number of concatenations performed is smaller
than in $P_{nc}$.
However, the cost of each 
concatenation is different due to
different sizes of the participating relations.
For example, $P_{nc}$ concatenates intermediate paths 
with $a$, $b$ and then $c$, while $P_{fc}$ does the same
with a single concatenation with cached $C_{abc}$.
In fact, depending on cardinalities of $|C_a|$, $|C_b|$, $|C_c|$, $|C_{bc}|$
$|C_{abc}|$, the concatenations performed in any
of the above plans might become the preferred cheaper alternative.

Further, the number of pruned tuples
in plans with or without caching
can significantly differ 
depending on the general shape of the graph.
For example, consider two basic graphs
$G_1$ and $G_2$ as presented in 
Fig.~\ref{fig:loop_caching_lensing}.
Both $G_1$ and $G_2$ have the same frequencies 
of labels $a$ and $b$,
but are different in terms of their \emph{shape}.
$G_1$ exhibits \emph{lensing} with focal points
on concatenations $b/a$, 
while $G_2$ has lensing in $a/b$.
Intermediate cardinalities of $\Delta^C$ (number of edge walks)
and $\Delta^R$ (number of pruned tuples)
of the \waveguide\ search are presented
for plans with ($P_{fc}$) and without ($P_{nc}$)
loop caching.
%
Observe that loop caching optimization is beneficial
for search in $G_1$ 
with 30\% and 33\% less edge walks and pruned tuples, 
respectively.
On the other hand, 
loop caching performs worse in $G_2$
with 92\% and 600\% more edge walks and pruned tuples,
respectively.
This can be explained by analyzing the edge walks and pruned tuples
during the concatenation sequence
$(\ldots/a/b)$ which is performed in $P_{nc}$, 
but not in $P_{fc}$.
In $G_1$, $(\ldots/a/b)$ computes a large number of intermediate
tuples most of which are later pruned due to a focal point in $b/a$.
Meanwhile, in $G_2$, $(\ldots/a/b)$ first prunes many tuples 
due to a focal point in $a/b$, 
hence reducing the total number of edge walks performed later in the search.

Lastly, we consider queries with constants.
In pipelined plan $P_{nc}$, 
this constant can be pushed to seed condition $S$ of its wavefront.
In fact, full concatenation $(abc)$ might not need to be ever computed in $P_{nc}$.
On the other hand, plans $P_{pp}$ and $P_{fc}$ allow at most partial constant pushdown,
since cached relations must be computed with universal seed to 
ensure completeness of the final closure.

\end{Sect}

%----------------------------------------------------------------------------%
\end{Sect}


==> eval.tex <==
%!TEX root = paper.tex
%============================================================================%
\begin{Sect}{Waveguide Plans}
\label{sec:eval}

\waveguide's evaluation strategy
is based on an \emph{iterative search algorithm}---%
and variations of it---%
which is guided by the \wgp s.
We are able to express complex query evaluation plans
which involve multiple search \emph{wavefronts}
that iteratively explore the graph.
%
The \emph{states} of the wavefront automata in a \wgp\
represent path queries in their own right.
As the \wgp\ (selectively) materializes states during evaluation---%
which we call \emph{path views}---%
this allows wavefronts to re-use intermediate results (paths)
that were already discovered by the search process.

%\begin{Sect}{Motivation}
%\label{sec:eval/motivation}
%
%We consider the differences between the two classes of algorithms we have discussed: 
%automaton-based and DP-based.
%%
%DP-based approaches have the advantage 
%of being similar in spirit to evaluation
%techniques used in relational databases. 
%There is a direct correspondence between the operator tree and 
%a query evaluation plan that is based on the relational algebra.
%Hence, 
%these algorithms can be implemented in most relational databases,
%thus inheriting the desirable features such as
%query evaluation planning, 
%execution pipelining, 
%avoiding re-computation by using materialized views,
%efficient indexing, 
%and robust external storage support. 
%However, 
%DP-based evaluation methods have several shortcomings, 
%which limit the opportunities for query optimization.
%The structure of evaluation plans is constrained 
%to trees in which
%branches are evaluated independently from each other. 
%In some cases, this leads to large intermediate result sets,
%which considerably slows down the evaluation process.
%To overcome this,
%sideways information passing (SIP, \cite{bancilhon1985magic}) strategies
%can be used as query rewrites of varying complexity:
%from classical selection push-downs\cite{ordonez2010optimization} to complex 
%strategies such as magic sets transformations\cite{seshadri1996cost}.
%Thus, the evaluation of even modest RPQs 
%may result in complex, highly-nested plans which are
%a challenge for present-day relational optimizers.
%
%Automaton-based methods address some of the shortcomings
%of DP-based approaches.
%Recall that query evaluation is performed by simultaneous traversal
%in the graph and the automaton, which recognizes a given regular expression.
%In other words, a search in a graph is \emph{controlled} by an automaton.
%Hence, an automaton can be considered a query evaluation plan.
%Since, in essence, an automaton is a type of a graph, 
%it follows that automaton-based methods have richer plan space 
%when compared to DP-based approaches. 
%Further, a path search in a graph with a shared state allows for 
%simpler sideways information passing between
%automaton sub-graphs responsible for evaluating different 
%parts of a regular expression. 
%Finally, a path search itself is not limited to breadth-first
%strategy. 
%In fact, 
%depth-first search or even hybrid adaptive strategy can be used instead. 
%Unfortunately, 
%automaton-based methods come with their fair share of serious shortcomings.
%For example, 
%as they are,
%none of these methods support external storage or indexing,
%which is a crucial requirement since real-life applications 
%often manage huge amounts of data.
%Further, in theory, automata enable rich evaluation planning,
%however, 
%in all of the algorithms, the controlling automaton is constructed 
%by following a bottom-up procedure based on the expression parse tree.
%This ensures that for each expression 
%at most single automaton can be constructed, 
%thus defying the purpose of evaluation planning.
%
%In this work, we aim to devise an RPQ evaluation strategy, 
%which is a hybrid of automata and DP-based approaches.
%We discuss our approach next.
%
%\end{Sect}
%

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
% why are FAs useful for us?

%It is natural, then,
%to consider how finite automata (FAs)
%could play a useful role in the evaluation of regular path queries.
%A corresponding FA could be used
%to {\em guide} the search in the graph for paths
%that establish answers for the query,
%and to {\em prune} effectively search that could not lead to answers.

%----------------------------------------------------------------------------%
\begin{Sect}{Wavefronts}
\label{sec:eval/overview}

% approach

In \waveguide,
we propose a novel strategy to perform efficiently
path search while \emph{simultaneously}
recognizing the path expressions.
%This approach is the fusion
%of two general evaluation strategies:
%	dynamic programming
%		and
%	\emph{iterative} search.
\waveguide's input is a graph database $G$
and a \emph{waveguide plan} (\wgp) $P_Q$
which \emph{guides} a number of search wavefronts
that explore the given graph.
%
% semi-naive (should we mention it here?)
This graph exploration, driven by an
iterative search procedure,
is inspired by the semi-na\"{\i}ve bottom-up
strategy used in evaluation of linear recursive
expressions based on \emph{fixpoint},
as is done for the \(\alpha\) operator for \ara,
described in \S\ref{SEC/bg/DP-based}.

The key idea is, given a \emph{seed} as a start,
to expand repeatedly 
the search wavefronts in the graph
until no new tuples are produced;
i.e., we reach fixpoint.
%
Each search wavefront is guided by a 
\emph{wavefront automaton},
a finite state machine based on 
non-deterministic finite automata (\nfa).
This is akin to the \fa\ approach discussed in \S\ref{SEC/bg/auto}.
Different, though,
from \nfa s which are used as recognizers 
of regular expressions on strings, 
wavefront automata introduce a number of features 
directed to evaluation of regular expressions
on graphs.
These include
	the use of \emph{seeds}, 
	\emph{append} and \emph{prepend transitions},
		and 
	\emph{path views}.

% In the following subsections we provide
% additional details as follows.
% 
First,
we present the iterative procedure used in \waveguide\
that drives the wavefront expansion.
Next,
we describe
the new types of transitions
enabled by the wavefront data-structure.
Finally,
we discuss
the interactions between different wavefronts
guided by a plan,
which can be used for optimization.

\end{Sect}
%----------------------------------------------------------------------------%
% Waveguide with QPA is an NFA
% * single wavefront search
\begin{Sect}{Expanding a Wavefront}
\label{sec:eval/expanding_a_wavefront}

% wfa features: seed by a constant
Each search wavefront has a \emph{seed} as its initialization. 
The seed is the set of nodes in the graph
from which this wavefront begins its search.
A seed can be either
\emph{universal} or \emph{restricted}.
A wavefront with a universal seed
conducts its search effectively starting
from \emph{every} node in a graph.
%On the other hand, 
A wavefront with a restricted seed
is restricted to starting search just from those nodes in its seed.
(A restricted seed will be defined by the results of other wavefronts or 
by constants used in a query.)
%
Graphically, 
a seed is represented as an incoming edge 
to starting state \state{q}[0]\ of the wavefront. 
We use the label ``\(U\)'' to denote a universal seed;
any other label on this edge denotes
a restriction placed on the seed,
thus a restricted seed.

Given an evaluation plan defined by search wavefronts,
the graph exploration is performed by an iterative procedure
as illustrated in Fig.~\ref{fig:direct_search_algo}.
%
% plan with a single wavefront
For example,
consider \wgp\ $P_1$
that uses a \emph{single} search wavefront 
to answer query $Q=(x,(ab)+,y)$ on graph $G$ 
as shown in Fig.~\ref{fig:eg_example_search}. 
Let the wavefront \(W_1\) be constructed by 
a direct mapping of the query's regular expression
into an \nfa.

% search cache
During the search, 
intermediate results are kept in a \emph{cache},
denoted at iteration \(i\) by \(C_i\).
This is a collection of tuples \tuple{u,v,\state{s}}\
for which \(u\) and \(v\) are nodes in \(G\)
and \state{s}\ is a state in \(W_1\).
% TODO: delta a set or a bag?
% should be a bag if we do partial reduce...
The newly discovered tuples found in the current iteration
are denoted by a \emph{delta} \(\Delta_i\).
%
We use the cache \(C_i\) and the delta \(\Delta_i\)
to eliminate intermediate answers we have already seen in the search.

% universal seed
In the first step of the search procedure,
all the universal seeds are initialized.
Specifically, \(\Delta^R_0\) is assigned
the set of \tuple{u,u,\state{q}[0]}\
for all \(u\in N\);%
\footnote{%
	This can be optimized to pull just the tuples
	from the triple store
	that can participate in the first step of any path to an answer.
	We call this \emph{first-hop} optimization.
}
\state{q}[0]\ is the starting state
for all wavefront automata with universal seeds.

%
% iterations
Next,
we loop over iterative steps.
In each iteration,
four operations are performed
	\textsf{seed},
	\textsf{crank},
	\textsf{reduce},
		and
	\textsf{cache}.
The iteration continues until fixpoint is reached.

\begin{figure}
    \begin{algo}
    \textsc[WaveguideSearch]($G, A_Q$)
    \end{algo}
    \begin{algo}[numbers=left,xleftmargin=0.5cm,numbersep=1pt]
     $\Delta_0^R\,\leftarrow\,$\textsf[seed]$(G)$; 
     $i\,\leftarrow\,0$;
     while $|\Delta_i^R|\,\geq\,0$ do
      $\Delta^S_[i+1]\,\leftarrow\,$\textsf[seed]$(\Delta^R_i)$;
      $\Delta^C_[i+1]\,\leftarrow\,$\textsf[crank]$(\Delta^S_[i+1],\,\Delta^R_i,\,G,\,C_i,\,A_Q)$;
      $\Delta^R_[i+1]\,\leftarrow\,$\textsf[reduce]$(\Delta^C_[i+1],\,\Delta^R_[i],\,C_i)$;
      $C_[i+1]\,\leftarrow\,$\textsf[cache]$(\Delta^R_[i+1],\,C_i)$;
      $i\,\leftarrow\,i+1$;
     done;
     \textbf[return] \textsf[extract]($C_i$);
    \end{algo}
    \caption{\waveguide\ evaluation procedure.}
    \label{fig:direct_search_algo}
\end{figure}

The \textsf{seed} step
populates the restricted seeds,
according to their respective seed conditions.
% TODO:
% if a seed is universal, then it is populated with all
% nodes in a graph, however this actually never happens because of 
% the first hop optimization..
% 17/12: we discussed universal seeds already - need an example for restricted seeds?
%
The \textsf{crank} step transitions
from the previous delta to the current,
$\Delta^R_i \rightarrow \Delta^C_{i+1}$.
%
For each node \(v\) in \(\tuple{u,v,\state{s}}\in\Delta^R_i\),
for edge \(\tuple{v,\state{a},w}\in G\)
and graph transition \(\tuple{\state{s},a,\state{t}}\in W\),
\tuple{u,w,\state{t}}\ is added to \(\Delta^C_{i+1}\).
Thus
\textsf{crank} advances the search \emph{simultaneously}
in the graph \emph{and} in the automaton.

To prevent unbounded computation over cyclic graphs,
the delta is \emph{reduced}:
\(\Delta^C_{i+1}\) is checked against
both the previous delta \(\Delta^R_i\)
and the cache \(C_i\);
tuples that are seen in either
\(\Delta^R_i\) or \(C_i\)
are removed to produce \(\Delta^R_{i+1}\).
%
Lastly,
the cache is updated \(C_{i+1}\)
by adding the tuples in the reduced delta \(\Delta^R_{i+1}\)
to it (\(C_{i}\)).
%
The iteration halts once \(\Delta^R\) is empty.

Recall $W_1$ in this example was produced
by directly mapping the regular expression \(r\)
% (from our query $Q$)
to an \nfa.
As the \nfa\ is a recognizer for \(r\),
it can be established by structural induction that,
for any tuple \(\tuple{u,v,\state{s}}\)
in the cache (\(C\))
such that \state{s}\ is an accepting state,
the pair of nodes \(\tuple{u,v}\)
must have a path between them in the graph
that conforms to \(r\).
Thus,
\waveguide\ produces the correct results.
%
The answer set can be then
\emph{extracted} from the cache
by selecting the tuples \(\tuple{u,v,\state{s}}\)
for all accepting states \state{s}\ of automaton \(W_1\).

% example: single wavefront search
% \textbf{Example 5.}
\begin{example} \label{EX single wavefront search}
Consider the wavefront search
in Fig.~\ref{fig:eg_example_search}
for a query with regular expression \(r = (ab)+\) on graph $G$.
Plan $P_1$ uses a single wavefront $W_1$ 
which is a basic wavefront embodying an \nfa\ that recognizes \(r\).

For each iteration $i$ of the search,
	cache \(S_i\),
	delta \(\Delta_i\),
		and
	reduced delta \(\Delta^R_i\)
are shown.
The search stops
when all newly generated tuples are, in fact,
duplicates, due to cycles in \(G\).
The cache tuples that are
in accepting state \state{q}[2]\ (shown shaded) are then
extracted as the answer set.
\end{example}
% example (end)

%From \(A_Q\),
%we can design a more efficient \qpa, \(P_Q\):
%	first,
%	compute \((ab)\);
%	then use a loop-back view transition
%	to compute the closure \((ab)+\).
%\(P_Q\) explores a smaller search space
%in fewer iterations than \(A_Q\)
%% not because of this! but, because of loop caching!
%because of the shorter cycle in the guiding automaton.
%In Fig.~\ref{fig:eg_example_search},
%for each iteration $i$ of the search,
%	cache \(S_i\),
%	delta \(\Delta_i\),
%		and
%	reduced delta \(\Delta^R_i\)
%are shown.
%The search stops
%when all newly generated tuples are, in fact,
%duplicates due to cycles in \(G\).
%The cache tuples that are
%in accepting state \state{q}[2]\ (shown shaded) are then extracted
%as the answer set.

\end{Sect}
%----------------------------------------------------------------------------%
\begin{Sect}{Guiding a Wavefront}
\label{sec:eval/guiding_a_wavefront}

% Waveguide with QPAs
% 
The construction of the \nfa\
forces an order to the query evaluation.
A ``wrong'' choice of \nfa\ can lead
to an inefficient evaluation plan.
%
In \waveguide,
we aim to minimize 
the search space explored
by considering the possible orders of graph exploration
by search wavefronts.
To achieve this,
we use wavefront automata
which can use transitions that
expand the wavefront
in the direction opposite to the direction
of the edges of the graph.

Consider a graph transition
\(\tuple{\state{s},l,\state{t}}\)
in wavefront $W$.
Edge label $l$ has a general form 
\prepend{a} or \append{a}, 
where $a$ is an edge label in $G$.
%
Position of a dot $\cdot$ 
specifies a direction of a search wavefront
and
denotes 
prepend (\prepend{a}) 
or 
append (\append{a})
transition. 
%
Prepend wavefront expands
in the opposite direction 
to the edges in the graph.
On the other hand,
append parameter guides a wavefront 
that expands in the same direction as the edges in the graph.
The semantics of \textsf{crank} operation on
prepend and append transitions 
are illustrated in Fig.~\ref{fig:eg_prepend_vs_append}.

% figure: example search
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{eg_nfa_execution.tikz}
	\caption{A run of waveguide plan $P_1$ over graph $G$.}
	\label{fig:eg_example_search}
\end{figure}

\begin{figure}
\centering
% figure: prepend vs append transition
\begin{subfigure}{\linewidth}
	\centering
	\includegraphics[width=\linewidth]{eg_prepend_vs_append.png}
	\caption{Prepending vs.~appending by expanding the wavefront using tuples from graph $G$.}
	\label{fig:eg_prepend_vs_append}
\end{subfigure}
% figure: graph vs view transition
\begin{subfigure}{\linewidth}
	\centering
	\includegraphics[width=\linewidth]{eg_graph_vs_view.png}
	\caption{Expanding the wavefront by appending and using the tuples from $G$ (over the graph) vs.~from search cache $C$ (over the view).}
	\label{fig:eg_graph_vs_view}
\end{subfigure}
\caption{Types of transitions used in a wavefront.}
\label{fig:transitions}
\end{figure}

Hence, wavefronts enable automaton transitions that explore the 
graph in a direction specified by the transition.
This allows to define a wavefront 
that can initiate evaluation from any label 
in the given regular expression
and iteratively expand by appending or 
prepending path labels.
This gives us the power to explore
all different expansion orders of
a single wavefront.

% crank over view (using the results of one wavefront in the other)
% seeding the wavefront

\end{Sect}
%----------------------------------------------------------------------------%
\begin{Sect}{Wavefront Interaction}
\label{sec:eval/wavefront_interaction}

%So far we have discussed how RPQs can 
%be evaluated by using a single search wavefront.
%If this wavefront is guided by an \nfa,
%then the order of expansion is effectively
%fixed by the way the \nfa\ was constructed,
%which might produce inefficient evaluation plans.
%To overcome this issue, 

Often, the search space is constrained even further
if several wavefronts are employed in the evaluation,
each evaluating parts of a given regular expression.
\waveguide\ enables this by defining
a number of automata,
one for each search wavefront.

% TODO: need more details on seeds..
%This allows to decompose a wavefront 
%Such seeds are useful in elimination
%of sub-path redundancy - an optimization we discuss later.

\waveguide\ plans,
in addition to transitions over graph edge labels, 
allow transitions over \emph{path views},
by utizing cached result sets produced by other wavefronts.
%hence, $W_1$ can \emph{expand} by using
%tuples computed by $W_2$. 
%
Consider a transition
\(\tuple{\state{s},l,\state{t}}\) in $W_1$.
If $a$ is an edge label in $G$, 
then this \emph{graph} transition expands the wavefront
by using the tuples from \emph{graph} $G$.
Otherwise, if $a$ is a state in $W_2$,
then this \emph{view} transition
expands the wavefront by employing the 
tuples produced by wavefront $W_2$
(as illustrated in Fig.~\ref{fig:eg_prepend_vs_append}).

These new types of transitions 
offer powerful choices in \wgp s
for guiding the search.
The search can have \emph{multiple} wavefronts 
originating from different starting points 
\emph{and} expanding in different directions.
% TODO: 
% this needs to be updated to seeds and combining wavefronts
%Wavefronts can be decomposed into sub-wavefronts 
%through seeding or 
Further, each wavefront can employ the cache
through transitions over views
to avoid unnecessary recomputation.%
\footnote{%
	This is also known as \emph{memoization}.
}

% example
% \textbf{Example 6.}
\begin{example} \label{EX view-wavefront}
Consider the wavefront search
in Fig.~\ref{fig:eg_example_search}
for a query \(Q\) with regular expression \(r = (ab)+\).
\(P_1\) is a basic \wgp\ embodying an \nfa\ that recognizes \(r\).
From \(P_1\),
we can design a more efficient \wgp, \(P_2\):
	first,
	compute \((ab)\) with wavefront $W_1$;
	then use a loop-back view transition
	to compute the closure \((ab)+\) (with wavefront $W_2$).
In this case, it can be shown that 
\(P_2\) explores a smaller search space
in fewer iterations than \(P_1\).
\end{example}
% (end) example

\end{Sect}
%----------------------------------------------------------------------------%
\begin{Sect}{The {\secsc Waveguide} Plan Space}
\label{sec:WGP space}

We claim that the space of waveguide plans
subsumes that of the \fa\ and \ara\ approaches,
as the Venn diagram in Fig.~\ref{fig:claim_img} shows
(and with the caveats as discussed in \S\ref{SEC/bg/plan_space}).

\begin{claim} \label{CLAIM subsumes}
\planspace[\wgp]\ \emph{properly subsumes} the union of
\planspace[\fa]\ and \planspace[\ara]\
(\(\planspace[\wgp] \supsetneq \planspace[\fa]\cup\planspace[\ara]\)).
\end{claim}

\noindent
That \planspace[\wgp]\ subsumes each of \planspace[\fa]\ and \planspace[\ara]\
is straightforward;
we devised \wgp\ so that we could express both \fa- and \ara- type plans.
\wgp\ extends the \fa\ model.
\wgp\ encompasses \ara\ by the addition of \emph{views};
what the \(\alpha\) operator offers,
transitive closure over an arbitrary relation,
can be accomplished by view-labeled transitions in a waveguide plan.

That \planspace[\wgp]\ properly subsumes
the union of \planspace[\fa]\ and \planspace[\ara]\
means that there is a waveguide plan that corresponds
to no \fa\ plan and to no \ara\ plan.
We have well demonstrated that in the discussions above.
Any \wgp\ with multiple wavefronts
and some wavefront with a long loop-back
is such a plan;
\fa\ plans are essentially single wavefront by the \fa\ model,
and pipelined loop-backs are outside the scope of \ara.
Likewise,
any \wgp, even single wavefront, that is ``mixed'',
that combines views and long loop-backs,
corresponds to no \fa\ plan and to no \ara\ plan.
(In Fig.~\ref{fig:loop_caching} on page \pageref{fig:loop_caching},
\(P_2\) with partial loop-caching is such a plan.)
%
Of course,
these very types of waveguide plans that \fa\ and \ara\ miss
often are the most efficient plans for a given query.

In \S\ref{sec:CoP},
we explain why this rich plan space is relevant.
In \S\ref{sec:experiments},
we we compare plans for real queries over real graph data
to establish that this is true in practice,
as well.

% In this section we show that plan space defined by \wfa s 
% $\mathcal{P}_{\text{WFA}}$
% is richer than both $\mathcal{P}_{\text{FA}}$
% and $\mathcal{P}_{\alpha \text{-RA}}$.

% % claim: FA subset of WFA
% \vspace{2mm}
% \noindent
% \textbf{Claim 3.}
% $\mathcal{P}_{\text{FA}} \subset \mathcal{P}_{\text{WFA}}$
% \\ 
% \noindent
% \textbf{Proof sketch:} Proceed with proof by construction. 

% % claim: a-RA subset of WFA
% \vspace{2mm}
% \noindent
% \textbf{Claim 4.}
% $\mathcal{P}_{\alpha\text{-RA}} \subset \mathcal{P}_{\text{WFA}}$
% \\ 
% \noindent
% \textbf{Proof sketch:} Again, proceed with proof by construction. 
% %

% % claim: FA subset of WFA
% \vspace{2mm}
% \noindent
% \textbf{Claim 5.}
% $\mathcal{P}_{\text{WFA}} \not\subset \mathcal{P}_{\text{FA}}$ and $\mathcal{P}_{\text{WFA}} \not\subset \mathcal{P}_{\alpha \text{-FA}}$
% \\ 
% \noindent
% \textbf{Proof sketch:} Proceed with proof by example. 

\end{Sect}
%----------------------------------------------------------------------------%
\end{Sect}


==> experiments.tex <==
%!TEX root = paper.tex
%============================================================================%
\begin{Sect}{Performance Study} 
\label{sec:experiments}

%----------------------------------------------------------------------------%
\begin{Sect}{The {\secsc Waveguide} Prototype} \label{sec:proto}

% (figure: example multiple wavefronts and interleaving)
\begin{figure}[t]
	\centering
	\includegraphics[width=0.72\linewidth]{system_overview.png}
	\caption{Overview of a prototype system}
	\label{fig:system_overview}
\end{figure}
% (end)

% To demonstrate the efficacy of the \waveguide\ evaluation strategy,
% we focus on evaluation of \sparql\ 1.1 property paths
% over large \rdf\ graphs.
% % Instead of providing an ad-hoc programmatical implementation
% % of the prototype,
% We illustrate how \waveguide\ can be implemented
% effectively on a modern relational database system.
% We use \postgresql\
% due to that it is open-source
% and has a high-performance procedural \sql\ implementation.
% However,
% any RDBMS with good procedural \sql\ support could be used.

We have prototyped a \waveguide\ system
that implements the methodology from \S\ref{sec:eval}
in order to benchmark waveguide plans to study their performance.
%
In this \waveguide\ system,
resource-intensive tasks are delegated to \postgresql\
via \sql\ and \emph{procedural} \sql\ routines.
This implementation
of our methodology provides
	high performance,
	scalability,
		and
	rapid deployment.

Fig.~\ref{fig:system_overview} shows the architecture.
It consists of two layers:
	\emph{application}
		and
	\emph{RDBMS}.
The application layer provides
	a user front-end,
	preprocessing the graph data,
	parsing user queries,
	generating \wgp s,
		and
	visualizing key steps during the search.
The RDBMS layer provides
	postprocessing of the graph data
		and
	performing the iterative \waveguide\ graph search
	for the given \wgp.

\end{Sect}
%----------------------------------------------------------------------------%
\begin{Sect}{Methodology}
\label{sec:experiments/methodology}

We test our implementation of \waveguide\ 
by running a collection of realistic path queries over real-world
datasets YAGO2s\cite{Yago2s} and DBPedia\cite{DBpedia}.
The datasets were preprocessed by removing invalid 
and duplicate triples and self-loops. 
After preprocessing, YAGO2s had 242M triples 
and DBPedia had 463M triples,
with 104 and 65K distinct predicates, respectively.
This makes these datasets 
well suited for benchmarking of path queries.

At the time of this paper,
we could not find any available benchmarks for 
\sparql\ property-path queries.
We therefore generate path queries based on 
data patterns we identified in real-world graphs. 
The goal of these experiments is to 
verify the gains offered by \waveguide\ optimizations,
and show that they correspond to the 
cost framework (\S\ref{sec:cost_framework}) 
and analysis (\S\ref{sec:cost_analysis}).

Our benchmark was executed on a 2xXeon E5-2640v2 CPU server 
with 7200RPM HDD running Ubuntu Server 12.04 x64 and PostgreSQL 9.3.  

\end{Sect}
%----------------------------------------------------------------------------%
\begin{Sect}{Threading}
\label{sec:experiments/threading}

%\begin{figure}[t]
%
%\centering
%\includegraphics[width=0.72\linewidth]{outliers.png}
%\caption{Outlier queries.}
%\label{fig:prod_cost}
%\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{prod_cost.png}
\caption{%
	Estimated cost of intermediate concatenations.
}
\label{fig:prod_cost}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{pruning.png}
\caption{Tuples pruned w/ \& w/o loop caching.}
\label{fig:bench_pruning}
\end{figure}

We benchmark the threading optimization by executing
a query of the following template pattern

\begin{prolog}[\sf]
	\qquad\qquad\=\kill
	\textsf{?x $p$/:locatedIn+/:dealsWith+ ?y}
	\plabel[Q locatedIn]{querynum}
\end{prolog}

\noindent
over the YAGO2s dataset,
with ``$p$'' as a variable predicate. 
We chose this template for the following reasons.
First, 
since \ref{Q locatedIn} contains
the concatenation of two transitive closures,
it is difficult to predict
the average length of the paths in the answer.
Second,
\textsf{locatedIn+} is a popular predicate
which also concatenates with many other predicates,
so there are many candidates for $p$.
Finally,
\textsf{locatedIn+} has an $\mathcal M$ value of $11.27$
which makes it a good candidate
for a threading split in $Q$.

We group $p$ candidates in two sets: 
the first (queries \textbf{L1}--\textbf{5})
having an $\mathcal M$ value greater than 10;
and
the second (queries \textbf{L6}--\textbf{14}) 
having an $\mathcal M$ value less than 1. 
Each of the queries is executed with three different plans:
	$D$, a direct evaluation with a single wavefront 
		with no threading;
	$T_1$ performs a threading split on predicate $p$;
	and
	$T_2$ threads on \textsf{locatedIn+}.

The relative running times for queries \textbf{L1}--\textbf{14}
executed with plans $D$ (the baseline), $T_1$, and $T_2$
are presented in Fig.~\ref{fig:threading_bench}.
%
As anticipated,
the evaluation of queries in the first group is
significantly (up to 75\%) faster threaded than direct,
and with $T_1$ being slightly faster than $T_2$.
This can be attributed to that the length
of the shared path $\mathcal L$ is shorter in $T_2$
due to a ``later'' threading split in the query expression.
%
Also as anticipated,
queries in the second group show bad results for $T_1$.
Indeed,
picking a predicate with $\mathcal M < 1$
for a threading split will generally be bad
due to few shared paths.
%
On the other hand, 
the results for $T_2$ are better than $D$
for 5 out of 9 queries in this second group.
This is explained by the lensing effect ,
which is produced by concatenation \textsf{$p$/:locatedIn+},
while $\mathcal M(G,p) < 1$ and 
$\mathcal M(G,\text{\textsf{:locatedIn+}}) > 10$.
%
Depending on whether
$\mathcal M(G,p/\text{\textsf{:locatedIn+}})$
is greater than or less than $1$,
threading is either desirable or not,
respectively.

\end{Sect}
%----------------------------------------------------------------------------%
\begin{Sect}{Loop Caching}
\label{sec:experiments/loop}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{edge_walks_vs_runtime.png}
\caption{%
	Edge walks vs.~runtime
	in plans w/ \& w/o loop caching
	in DBPedia.
}
\label{fig:edge_walks_vs_runtime}
\end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{threading_bench.png}
\caption{Threading over YAGO2s.}
\label{fig:threading_bench}
\end{figure}

% figure: benchmark results
\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{bench.png}
	\caption{Effect of plans on query evaluation.}
	\label{fig:bench}
\end{figure*}

We benchmark the loop-caching optimization 
by executing a collection of queries
of the simple template $Q_{(ab)+} = (x, (ab)+, y)$
(\ref{Q AB+})
with two \wgp s $P_{nc}$ and $P_{fc}$,
which specify executions of $Q$ with no loop caching 
and with full loop caching, respectively.

Values for $a$ and $b$ were chosen
by iterative pruning of predicates 
appearing in the DBPedia dataset.
First,
we excluded predicates with very high 
(more than 25M) and low (less than 75K)
cardinalities.
Then,
we ran query $Q_{abab} = (x, (abab), y)$ 
and recorded those $(a,b)$ predicate pairs 
for which the result of $Q_{abab}$ was not empty.
DBPedia had 1171 such pairs,
which indicates a high number of 
$(ab)+$ paths in this dataset.
For each of these pairs,
we ran the full closure query $Q_{(ab)+}$
to obtain its \emph{expansion ratio},

\begin{prolog}
	\(r_{\text{exp}} = \frac{|Q_{(ab)+}|}{|Q_{ab}|}\)
	\plabel[EQ ratio]{eqnum}%
\end{prolog}

\noindent
where $|Q|$ denotes the cardinality of a query result.

Recall that both $P_{nc}$ and $P_{fc}$
initially evaluate $(ab)$ paths in the same way,
while the rest of the closure $(ab)+$ is computed differently. 
Hence,
in order to show the differences 
between these plans,
we chose predicate pairs with $r_{\text{exp}} \gg 1$,
so that the computation of the rest of the closure constitutes 
the majority of the plan execution time.
We identified 38 such queries
by analyzing graph patterns in DBPedia. 

We evaluated each one of these queries with 
$P_{nc}$ and $P_{fc}$ plans and recorded
the \emph{running time}, \emph{edge walks} and \emph{pruning statistics}.
Due to widely varying absolute values for these
statistics across queries,
we present their relative percentage breakdowns
in Fig.~\ref{fig:edge_walks_vs_runtime}, as follows.
Each query is represented by a two-colored bar,
which shows the percentage breakdown of statistics values
between $P_{nc}$ and $P_{fc}$ executions.
%
In this way, 
we present edge walks (in the left chart)
and running-time execution (in the right chart).
We enumerate the queries from \textbf{D1} to \textbf{D38}
according the ascending sorting of 
the percentage of edge walks 
performed in the $P_{nc}$ execution relative to the $P_{fc}$ execution.
Hence,
in query \textbf{D1}, 
$P_{nc}$ execution resulted in significantly 
fewer edge walks relative to $P_{fc}$ execution,
with the opposite true for query \textbf{D38}.
Finally,
we perform a further breakdown,
for each query, 
of the total number of edge walks into 
	the number of tuples which were cached, 
	were reduced against the cache,
	or 
	were reduced against the delta.
This breakdown is represented by different 
shades of the color associated with $P_{nc}$ or $P_{fc}$
executions, respectively.

Our first observation is that, in general,
the loop caching optimization can
significantly increase \emph{or} decrease the total
number of edge walks performed by the search.
In our benchmark,
loop caching resulted in fewer edge walks in 
68\% of the queries,
with almost an order of magnitude reduction,
in the best case.
On the other hand,
in 32\% of the queries,
loop caching resulted in more edge walks, 
with a more than 5X increase,
in the worst case.

Our second observation is that the query running time 
is correlated to the total number of edge walks performed,
but with some deviations.
In queries with bad loop caching performance
(\textbf{D1}-\textbf{D8}), 
the running time grows more slowly
than the number of edge walks. 
This is due to that,
in these queries,
the majority of edge walks produced duplicate tuples,
which were removed against the delta.
Such removals are inexpensive,
as discussed in \S\ref{sec:cost_framework}.
On the other hand, 
due to the lack of delta removals in edge walks,
we observe an increase in the running time
relative to the number of edge walks
in \textbf{D17, D20, D24-31}, and \textbf{D33-34}.
%
The running time for outliers \textbf{D8} and \textbf{D38}
is affected by the cost of intermediate concatenations
performed during the evaluation.
Simple cost estimates
(based on the product of relations) 
for \textsf{crank}s over iterations are presented 
in Fig.~\ref{fig:prod_cost}.
In \textbf{D8},
$|C_{ab}| \gg |C_a|$ and $|C_{ab}| \gg |C_b|$,
which slows down the concatenations
in $P_{lc}$ when compared to $P_{nc}$.
The opposite is observed in \textbf{D38},
yielding the advantage to $P_{fc}$ over $P_{nc}$. 

Lastly,
we study the effect of lensing
by analyzing the degree
of \textsf{delta} and \textsf{cache} pruning.
% over iterations of the search.
Fig.~\ref{fig:bench_pruning} plots pruning 
over iterations for the queries which exhibit lensing:
\textbf{D3} and \textbf{D38}.
Query \textbf{D3} has $\mathcal M(G,a)=10.58$ and $\mathcal M(G,b)=0.33$,
which suggests lensing with focal point on the concatenation $a/b$.
As discussed in \S\ref{sec:cost_analysis},
this can significantly increase amount of pruning
for loop caching,
which is indeed what we observe.
%
On the other hand,
\textbf{D38} has $\mathcal M(G,a)=0.07$ and $\mathcal M(G,b)=5.34$,
which suggests lensing with focal point on the concatenation $b/a$.
This lensing benefits loop caching 
by decreasing the amount of pruning over iterations,
which is what we observe.

\end{Sect}
%----------------------------------------------------------------------------%
\begin{Sect}{Combined Optimizations}
\label{sec:experiments/mixed}

%%----------------------------------------------------------------------------%
%\begin{Sect}{Implementation} \label{sec:imp}
%%
%We implement our \waveguide\ prototype
%as an application over the \postgresql\ relational database.
%The ``application'' layer provides
%	a user front-end,
%	preprocessing the graph data,
%	parsing user queries,
%		and
%	generating \qpa s.
%The graph search itself
%is encoded as \emph{procedural} \sql\ routine,
%which is executed by the database system.

%\end{Sect}
%----------------------------------------------------------------------------%
%\begin{Sect}{Illustration} \label{sec:illus}

We illustrate the impact of combining
\waveguide\ optimizations
%Due to limited space,
over the example query

\begin{prolog}[\sf]
	\qquad\qquad\=\kill
	\textsf{?p :marriedTo/:diedIn/:locatedIn+/:dealsWith+ USA}
	\plabel[Q diedIn]{querynum}
\end{prolog}

\noindent
over the YAGO2s dataset. 
We instantiate \textsf{p} as follows.

\begin{itemize}
\item [{\pathQ[1]}:]
	single wavefront \textsf{USA} $\rightarrow$ \textsf{?p}.

\item [{\pathQ[2]}:]
	single wavefront \textsf{?p} $\rightarrow$ \textsf{USA}.

\item [{\pathQ[3]}:]
	two wavefronts

	\begin{center}
	\textsf{?p} $\rightarrow$ \textsf{:locatedIn+/:dealsWith}
		$\leftarrow$ \textsf{USA}.
	\end{center}

\item [{\pathQ[4]}:]
	\pathQ[2]\ but with a threaded sub-path

	\begin{center}
	\textsf{:locatedIn+/:dealsWith+ USA}.
	\end{center}

\end{itemize}

\noindent
Fig.~\ref{fig:bench}a shows the effect
of wavefront choice on search cardinality. 
Note the order of magnitude difference between 
the best, \pathQ[4],
versus the worst, \pathQ[1].
%
The three types of redundancy pruning---%
	\textsf{cache},
	\textsf{delta},
		and
	\textsf{fpp}---%
are illustrated for each plan.
Fig.~\ref{fig:bench}b plots
search size across iterations for \pathQ[2]\
with pruning;
over \(40\%\) of tuples are pruned!
%
Fig.~\ref{fig:bench}c plots
delta sizes over iterations
for \pathQ[1]\ and \pathQ[3].
%
Note how the selective search of \pathQ[3]\ is better behaved 
than the rapid expansion of \pathQ[1].
%
In Fig.~\ref{fig:bench}d,
the total execution time
for each plan is presented.
%
This demonstrates the significant improvement in performance
achievable by careful design of the \wgp.

\end{Sect}

%----------------------------------------------------------------------------%
\end{Sect}


==> intro.tex <==
%!TEX root = paper.tex
%============================================================================%
\begin{Sect}{Introduction} \label{sec:introduction}
%----------------------------------------------------------------------------%
% Motivation

Graph data is becoming rapidly prevalent
with the rise of the Semantic Web,
social networks,
and data-driven exploration in life sciences.
There is need
for natural and efficient ways to query
over these graphs.
%%% ...

The Resource Description Framework (\rdf)
\cite{rdf}
provides a data model for graph data.
An \rdf\ \emph{store} is a set of \emph{triples}
that describes a directed, edge-labeled multi-graph.
A triple, \tuple{\subject, \role, \object},
denotes an \emph{edge}
from \emph{node} ``\subject''
	(the \emph{subject})
to node ``\object''
	(the \emph{object}),
with the edge labeled by ``\role''
	(the \emph{role},
	also called as the \emph{label} or as the \emph{predicate}).%
\footnote{%
	The object in an \rdf\ triple is allowed to be a \emph{literal}
	as well as a node.
	However, this distinction is not important for us.
}

Correspondingly,
the \sparql\ query language
\cite{prud2008sparql}
provides a formal means to query over \rdf\ stores.
A query defines sub-graph match criteria;
its evaluation over an \rdf\ store returns
all embedded sub-graphs meeting the criteria.
%
For example,
the query
	``\textsf{?friend :friendOf Charles}''
evaluates to a list people
	(nodes, binding to variable ``\textsf{?friend}'')
who are friends of
	(role ``\textsf{:friendOf}'')
``\textsf{Charles}''
	(a named node, so a constant).
This is a simple query, of course,
and could be evaluated just by extracting the triples
with
	``\(\mbox{\textsf{r}} = \mbox{\textsf{:friendOf}}\)''
and
	``\(\mbox{\textsf{o}} = \mbox{\textsf{Charles}}\)''.
%
For even an only slightly more complicated query,
however,
it may not be straightforward
to find a \emph{plan}
to evaluate it efficiently.

In its current version, 1.1,
\sparql's expressiveness
has been extended
with \emph{property paths}
\cite{harrissparql}.
Instead of specifying
the path of interest \emph{explicitly} between nodes,
one may now specify it \emph{implicitly}
via a \emph{regular expression}.
(This also means matching paths in the graph
are not bounded in length by the query's expression,
while they are in \sparql\ 1.0).
%
For example,
the query
	``\textsf{?friend :friendOf+ Charles}''
evaluates to a list people
who are friends of ``\textsf{Charles}'',
or
friends of people who are friends of ``\textsf{Charles}'',
and so forth.%
\footnote{%
	``\textsf{:friendOf+}'' represents the \emph{transitive closure}
	over edges labeled as ``\textsf{:friendOf}''.
}

Property paths effectively introduce
the concept of \emph{regular path queries} (\rpq s)---%
well studied before the advent of \rdf\ and \sparql---%
into the query language.
%
% An \rpq\ matches pairs of nodes,
% such that each pair is connected by a path in the graph
% matching the query's \emph{regular expression}.
%
While eminently useful,
such queries are even more challenging
to optimize well.
%
% We have embarked on a long-term project
% called \waveguide\
% to build a highly effective, full-fledged cost-based optimizer
% for \sparql\ queries that use property paths.
%
We have embarked on a long-term project
called \waveguide\
with the ultimate goal
to provide viable cost-based query optimization
and evaluation for \sparql\ over \rdf\ stores
that is on par
with the state of the art for relational database systems.

%----------------------------------------------------------------------------%
% Objectives

% In this paper,
We address the critical first step of this endeavor,
defining a rich \emph{plan space}---%
the space of \emph{waveguide plans} (\wgp s)---%
for \sparql\ queries.
% DISCLAIMERS...
We focus on single-path, property-path queries,
essentially the \rpq\ fragment of \sparql\ 1.1.
We consider a set semantics---%
the \textsf{distinct} directive in each query---%
and thus do not consider aggregation.
%
Contributions of this work are as follows.

\begin{enumerate}
\item \label{contrib:plans}
	\emph{Waveguide-plan space}.

	\begin{enumerate}
	\item \label{contrib:summarize}
		\emph{Summarize}
		the state of the art for evaluation of \rpq s
		and \sparql\ property paths
		(\S\ref{SEC/bg}).
		\emph{Establish}
		why none suffices
		(\S\ref{SEC/bg/plan_space}).

	\item \label{contrib:subsumes}
		\emph{Devise}
		the waveguide place space
		(\S\ref{sec:eval}).
		\emph{Demonstrate}
		it \emph{subsumes} the state of the art,
		and extends well beyond it
		(\S\ref{sec:WGP space}).

	\item \label{contrib:opt}
		\emph{Model} the \emph{cost factors}
		that determine the efficiency of plans
		(\S\ref{sec:CoP}).
		\emph{Present}
		the powerful optimizations
		offered by waveguide plans
		(\S\ref{sec:methods}).

	\end{enumerate}

\item \label{contrib:performance}
	\emph{Performance study}.

	\begin{enumerate}
	\item \label{contrib:prototype}
		\emph{Provide}
		an evaluation framework
		(\S\ref{sec:proto}).

	\item \label{contrib:benchmark}
		\emph{Benchmark}
		query plans for realistic queries over real \rdf\ stores / graphs
		(\S\ref{sec:experiments}).
%
% 	\item \label{contrib:substantiate}
		\emph{Substantiate} the optimizations
		of our approach
		(\S\ref{sec:experiments/threading},
		\S\ref{sec:experiments/loop}, \&
		\S\ref{sec:experiments/mixed}).

	\item \label{contrib:necessity}
		\emph{Justify} the \emph{necessity}
		of planning and the waveguide plan space
		(\S\ref{sec:experiments}).

	\end{enumerate}

\end{enumerate}

% Within our framework,
% a query plan---%
% called
A \emph{waveguide plan} 
% (\wgp)---%
consists of
	a collection of (non-deterministic) finite automata
	for the property path and
	search directives
which \emph{guides} the query evaluation.
%
In \cite{YGG2015:eval},
we demonstrated that,
with proper choice of plan,
we can gain orders of magnitude performance improvement
for many property-path queries over real datasets,
while maintaining comparable performance for other queries,
as the leading \sparql\ query engines
as \jena\
\cite{ApacheJena2013}
and \virtuoso\
\cite{erling2010virtuoso}.
%
We evince that planning is critical
to evaluate \sparql\ queries efficiently,
and that choosing the right plan depends on the underlying graph data
and thus ultimately must be cost-based.

%%% ...

% A \sparql\ path query can be potentially evaluated
% by any number of \wgp s.
% A number of objectives must be balanced within a query plan;
% thus,
% this is a multi-objective optimization problem.
% We propose a cost-based method
% that selects the best \wgp\
% based on its estimated total cost.
% Our ultimate goal
% is a cost-based optimizer for \sparql\ queries for \rdf\ databases
% of the same caliber
% as cost-based optimizers
% for \sql\ queries for relational databases.

%----------------------------------------------------------------------------%
% Contributions & Outline

% We summarize the main contributions of this work as follows:

% \begin{itemize}
% \item
% 	We devise a framework for evaluation of regular path queries
% 	based on iterative search in the graph guided
% 	by automata-based wavefront plans;

% \item
% 	Based on the benchmark on real graph datasets,
% 	we identify the factors specific to RPQ evaluation
% 	that can magnify the query cost;

% \item
% 	Based on these cost factors,
% 	we outline the number of novel optimization methods
% 	that are enabled by our wavefront plans. 

% \end{itemize}

% In Section \ref{sec:eval},
% we introduce \waveguide's evaluation strategy (\emph{run-time}),
% and the \emph{query plan automata} (\emph{compile-time})
% used to guide the evaluation.
% %
% In Section \ref{sec:CoP},
% we
% 	overview a \emph{cost model} for \wgp s,
% 	discuss \emph{search cost factors} that influence evaluation efficiency,
% 		and
% 	enumerate \emph{optimization methods} that address these.
% %
% In Section \ref{sec:experiments},
% we briefly present the architecture of our present \waveguide\ prototype,
% and illustrate the viability of \wgp s with the optimization methods
% with an example query 
% over the YAGO2s \cite{Yago2s} \rdf\ dataset.
% %
% In Section \ref{sec:conc},
% we enumerate our next steps,
% and conclude.

%----------------------------------------------------------------------------%
\end{Sect}

